Model-Free Generative Replay for Lifelong Reinforcement Learning: Application to Starcraft-2

One approach to meet the challenges of deep lifelong reinforcement learning (LRL) is careful management of the agent's learning experiences, to learn (without forgetting) and build internal meta-models (of the tasks, environments, agents, and world). Generative replay (GR) is a biologically inspired replay mechanism that augments learning experiences with self-labelled examples drawn from an internal generative model that is updated over time. We present a version of GR for LRL that satisfies two desiderata: (a) Introspective density modelling of the latent representations of policies learned using deep RL, and (b) Model-free end-to-end learning. In this paper, we study three deep learning architectures for model-free GR, starting from a na\"ive GR and adding ingredients to achieve (a) and (b). We evaluate our proposed algorithms on three different scenarios comprising tasks from the Starcraft-2 and Minigrid domains. We report several key findings showing the impact of the design choices on quantitative metrics that include transfer learning, generalization to unseen tasks, fast adaptation after task change, performance wrt task expert, and catastrophic forgetting. We observe that our GR prevents drift in the features-to-action mapping from the latent vector space of a deep RL agent. We also show improvements in established lifelong learning metrics. We find that a small random replay buffer significantly increases the stability of training. Overall, we find that "hidden replay" (a well-known architecture for class-incremental classification) is the most promising approach that pushes the state-of-the-art in GR for LRL and observe that the architecture of the sleep model might be more important for improving performance than the types of replay used. Our experiments required only 6% of training samples to achieve 80-90% of expert performance in most Starcraft-2 scenarios.

==> SRI CoLLA 2022 L2M Paper Revised/abstract.tex <==
% The challenge of reinforcement learning on a sequence of tasks presented throughout an agent's lifetime is known as lifelong reinforcement learning (aka continual reinforcement learning (RL)). 
One approach to meet the challenges of deep lifelong reinforcement learning (LRL) is careful management of the agent's learning experiences, in order to learn (without forgetting) and build internal meta-models (of the tasks, environments, agents, and world).
Generative replay (GR) is a biologically-inspired replay mechanism that augments learning experiences with self-labelled examples drawn from an internal generative model that is updated over time. %The generative model is also updated on-the-fly.
We present a version of GR for LRL that satisfies two desiderata: (a) Introspective density modelling of the latent representations of policies learned using deep RL, and (b) Model-free end-to-end learning. 
%\sout{The first property avoids the challenges of density modelling of complex high-dimensional perceptual inputs, whereas policy learning using deep RL works well with such perceptual inputs. 
%The second property avoids the challenges of learning temporal dynamics and reward functions from few learning experiences with sparse rewards. }
In this paper, we study three deep learning architectures for model-free GR, starting from a na\"ive GR and adding ingredients to achieve (a) and (b). 
We evaluate our proposed algorithms on three different scenarios comprising tasks from the \SC{} and Minigrid domains.
We report several key findings showing the impact of the design choices on quantitative metrics that include transfer learning, generalization to unseen tasks, fast adaptation after task change, performance comparable to a task expert, and minimizing catastrophic forgetting.  
We observe that our GR prevents drift in the features-to-action mapping from the latent vector space of a deep RL agent. 
We also show improvements in established lifelong learning metrics. 
We find that a small random replay buffer significantly increases the stability of training when combined with the experience replay buffer and the generated replay buffer.
% continual learning when GR is combined with ER within a dual memory learning system that operates in ``wake-sleep'' phases, where sleep phases use policy distillation on the GR+ER replay buffer, and wake phases leverage the policy for off-policy RL in a new task.  
Overall, we find that ``hidden replay'' (a well-known architecture for class-incremental classification) is the most promising approach that pushes the state-of-the-art in GR for LRL, and observe that the architecture of the sleep model might be more important for improving performance than the types of replay used. Our experiments required only 6\% of training samples to achieve 80-90\% of expert performance in most \SC{} scenarios.

% significantly improves upon na\"{i}ve single-task RL and other replay architectures.
% We evaluate our proposed algorithms using a suite of lifelong RL metrics on a diverse set of scenarios comprising tasks from the \SC{} and Minigrid domains, and we find that ``hidden replay'' (a well-known architecture for class-incremental classification) significantly improves upon na\"{i}ve single-task RL and other replay architectures.
%: (a) We demonstrate that single task learning using wake-sleep phases converges to optimal policies. (b) The benefit of generative replay can depend on careful choice of architecture. We conduct 
%We evaluate our approach empirically on a suite of lifelong learning metrics using a diverse set of lifelong RL scenarios comprising tasks from the \SC{} and Minigrid domains. 
%We compare several instantiations of the framework with different architectures and find that using ``hidden replay'', a technique that has been successful in supervised classification, significantly improves upon na\"{i}ve non-lifelong RL. 
% \sout{Building upon this framework, we make the rather unique contribution of integrating 
% %multiple integrated lifelong RL systems that incorporate 
% multiple independently-developed lifelong learning components.
% %within our wake-sleep framework.
% We evaluate using a suite of lifelong RL metrics on a diverse set of scenarios comprising tasks from the \SC{} and Minigrid domains.}
% \sout{We show empirical gains from adding: adaptive sleep triggered by changepoint detection; compression of experiences using quantization; prioritized replay using continual danger detection; unsupervised/self-supervised representation learning of observation; and mixture modeling of disparate tasks using multiple generative models. Our integrative approach highlights the prospect of easier system integration enabled by lifelong learning components.}
%Our work makes several empirical contributions. i.) We demonstrate that single task learning using wake-sleep phases converges to optimal policies. ii.) The benefit of generative replay can be higher with careful choice of architecture. We conduct a thorough investigation of three different replay architectures, with the finding that ``hidden replay'' (a well-known replay architecture for supervised classification) dominates in the lifelong RL setting as well. Our subsequent contributions investigate lifelong learning agents in the game of Starcraft-2. We integrate recently published continual learning algorithms within the context of wake-sleep phases, and report that the following combinations lead to improved lifelong RL iii.) sleep phase triggered in an adaptive manner using continual changepoint detection, iv.) compression of experiences using continual tensor quantization, v.) prioritized replay using continual danger detection, and vi.) mixture modelling of disparate tasks using multiple generative models. Our empirical results are over lifetimes of RL tasks defined in Starcraft-2 and Minigrid. Since deep learning in Starcraft-2 is computationally demanding, we release a dataset  generated by single task experts in order to enable future research. Our comprehensive results show improved performance over non-lifelong agents in terms of established quantitative metrics for lifelong learning, and shows the prospect of easier system integration of  lifelong learning components.

==> SRI CoLLA 2022 L2M Paper Revised/discussion.tex <==
\section{Discussion}

% In this paper, we have presented the results of a multi-year multi-university collaboration to better understand wake-sleep based lifelong RL systems, new replay methods for lifelong RL, improved representation learning for generalization, and improved agents for \SC{}. Our experiments demonstrate lifelong learning via positive forward and backward transfer, high performance policies relative to single task expert, and reduced catastrophic forgetting. 

Our experiments demonstrate LRL via positive FT and BT, high performance relative to an STE, reduced catastrophic forgetting, and fast adaptation to new tasks. Our work clearly advances the domain-specific state-of-the-art in \SC{} by reducing the sample complexity of deep RL to master the minigames.
Compared to STE, our experiments required only 6\% of training samples to achieve 80-90\% of expert performance. 
Existing lifelong RL implementations (e.g., \citep{mendez2020lifelong}) have been tested on benchmark problems, but proved to be challenging to scale up to the complex observation and action space of SC-2. Future work can leverage our techniques in the full SC-2 game and reduce the astronomical sample complexity of current deep RL agents in SC-2 (e.g., AlphaStar \citep{vinyals2019grandmaster}). 

While the wake-sleep mechanism and model-free GR show promising results, there is room for improvement, and the approach is easily extensible. We highlight several potential extensions. Our current model triggers sleep on a set schedule. Instead, it is possible to self-trigger sleep via recent work in lifelong changepoint detection \citep{faber2021watch}. Currently, we store full observations in the replay buffer, which due to memory constraints, limits the number of samples that can be saved. It would be prudent to intelligently compress experiences in the replay buffer \citep{riemer2019scalable, wang2021acae, caccia2020online,zhang2017deeper,schaul2015prioritized, hayes2019remind}. Past work has looked at improving replay buffers via prioritized replay \citep{schaul2015prioritized} based on detecting dead-end states. 
We further hypothesize that increasing the lifetime of an agent by avoiding dead end states is a useful bias. Our methods operate over hand-crafted representations of the observation space; the system could be extended by introducing representation learning from RGB-observations via unsupervised (STAM \citep{smith2019unsupervised,smith2019unsupervised2}) and self-supervised learning \citep{gallardo2021self}. We can further extend our models using mixtures of VAEs (e.g., the Eigentask framework \cite{raghavan2020lifelong}) to dynamically grow and shrink the model, leading towards agents that build implicit models of the tasks they experience. Finally, we used a fixed neural architecture and loss functions throughout the agent's lifetime. GR is a flexible approach that can include progress in other areas of lifelong learning, e.g., dynamically changing the underlying neural architectures \citep{schwarz2018progress}, neuromodulation \citep{brna2019uncertainty}, and regularization \citep{kolouri2019sliced}. 
Further, interesting avenues include the application of GR to multi-agent RL \citep{nekoei2021continuous} and federated learning \citep{rostami2017multi}, where communication between agents can enable better coordination between agents and collective acquisition of knowledge. Due to the inherent plastic-yet-stable nature of lifelong learners, our methods can be more robust to data drift, concept drift, or task changes, reducing system downtime and the overhead of retraining, and used to address  model obsolescence and reduce the technical debt of machine learning models \citep{sculley2015hidden, alahdab2019empirical, bogner2021characterizing}. 

% \sout{In addition to the basic studies presented in this paper, we also explored the integration of the aforementioned lifelong learning components within the context of  wake-sleep via a multi-year multi-university collaboration using the \SC{} domain, and showed the framework to be sufficiently expressive. Preliminary experiments suggest that the addition of each component can result in improved lifelong learning (see Section \ref{app:system}).}

% Since deep learning in \SC{} is computationally demanding, we release a dataset generated by single task expert policies, and we make it publicly available for future research.

% In these experiments, we used a fixed neural architecture and loss functions throughout the agent's lifetime. However, generative replay is a flexible approach that can potentially include additional lifelong learning techniques such as dynamic changes to the underlying neural architectures \citep{schwarz2018progress}, neuromodulation \citep{brna2019uncertainty} and regularization \citep{kolouri2019sliced}. For example, the Eigentask framework \cite{raghavan2020lifelong} can be extended to dynamically grow and shrink the number and task-subtask relationships between the Eigentasks, heading towards agents that can build an implicit model of the tasks they experience. Future work can build on our work to explore these ideas within the wake-sleep framework. 
 %Future work can build on our work to explore these ideas within the wake-sleep framework. 




==> SRI CoLLA 2022 L2M Paper Revised/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Evaluation scenarios}
\label{sec:scenarios}
A lifelong learning \textit{scenario} describes the order of task presentation and repetition of tasks. A concrete instantiation of a scenario with tasks (or POMDPs) is called a \textit{syllabus}. Each scenario is used to evaluate the learning agent over all syllabi and average metrics. The three  scenarios we consider are depicted in Figure~\ref{fig:scenarios}.
 \textbf{Pairwise:} Two tasks are presented once each. This scenario evaluates knowledge transfer between two tasks. \textbf{Alternating:} Two tasks are presented with three repetitions of each pair. This scenario evaluates knowledge retention over longer lifetimes. \textbf{Condensed:} A random permutation of all tasks is presented. 
 % Task variants appear after all tasks have been seen once. 
 This is a useful setting for understanding how an agent performs across different task orderings.
 
Given a syllabus, an experiment run alternates between \emph{evaluation blocks} (EBs) and \emph{learning blocks} (LBs) \citep[see][]{new2022lifelong}. 
We say that a task is \emph{seen} wrt an EB if it has appeared in any LB preceeding it, otherwise it is \emph{unseen}.
During each EB, the average accumulated reward of the agent is evaluated on all tasks in the syllabus (including unseen tasks); during each LB, the agent learns on a single task for a fixed number of interactions. 
The STE for each task serves as a baseline and measures the relative performance of the learner wrt asymptotic optimal.

\subsection{Metrics for Lifelong RL}
% To understand the relative merits of our algorithm, w
We run controlled and quantitative experiments and compare to multiple baselines along three sets of metrics. 
First, we compare learning behavior by examining the accumulated rewards captured by periodic evaluations of the agent, i.e., we look at the trend of EB rewards averaged over EBs (and tasks). 
% for all tasks in a syllabus.
Second, we aim to understand how the rewards achieved by an agent compares to 
%the ``optimal'' policy by comparing to the terminal performance of agents trained on each task to convergence (
a single task expert (STE). 
This forms the basis for our second set of metrics: \emph{relative reward (RR)}.
%to the terminal reward achieved by a single task expert. 
Note that these metrics also focus on 
% purely on understanding the dynamics of 
EBs and do not consider  % fast adaptation in 
LBs. Finally, we compare algorithms using the lifelong learning metrics defined by \citep{new2022lifelong}, which take into account both LBs and EBs, and aim to frame metrics in a way that are agnostic to the domain.

We begin by describing the RR metrics. 
% , which always frame the metrics in the context of performance compared to a well-trained single task expert. 
For each task, we train (offline) the STE % \textit{single task expert (STE)}, 
using an off-the-shelf deep RL algorithm. % for a single task, to convergence. 
% We develop a set of metrics comparing the performance of an agent at each evaluation block to the terminal performance of the STE in order to identify how well the agent has
RR metrics measure how well the agent has learned the seen tasks, how well the agent performs over all tasks in the syllabus, and how well the agent generalizes to unseen tasks. 
In general, RR is computed as
\begin{align}
RR(\pi,T,S) &= \frac{1}{|T|}\sum_{t \in T}\frac{1}{|S(t)|}\sum_{s \in S(t)} \frac{r_\pi(s)}{r_{\pi^*_s}(s)} 
\label{eq:rr}
\end{align}
where $\pi$ is the policy of the learner, $T$ is a set EBs, $S(t)$ is the set of tasks at EB $t$, $\pi^*_s$ is the STE for  task $s$, and $r_{\pi}(s)$ is the accumulated reward (return) achieved on task $s$ from using policy $\pi$. Different metrics are defined by setting $S, T$ to different EBs and tasks. 

$\mathbf{RR_\Omega}$: $T$ only includes the final EB, and $S(t)$ is the set of  seen tasks in the syllabus. $RR_\Omega$ measures how well the agent has learned the seen tasks in the syllabus ``at the end of the day''. To measure catastrophic forgetting, we denote $\mathbf{RR_\sigma}$ where 
$T$ includes all EBs, and $S(t)$ is the set of seen tasks in the syllabus encountered in previous LBs up to and including EB $t$. $\mathbf{RR_\upsilon}$ is complementary in that it measures how well the agent generalizes to unseen tasks, $T$ includes all EBs, and $S(t)$ is the set of unseen tasks not encountered in previous LBs up to and including EB $t$. To measure plasticity, we denote $\mathbf{RR_\alpha}$ where $T$ is the set of all EBs, and $S(t)$ is only the task learned in LB $t$ preceeding EB $t$.
Note that in all cases, higher more-positive values are better for all metrics as all our STEs achieve positive return.

% We define the following metrics: \textbf{Relative reward in the final EB (RR\textsubscript{$\Omega$}):} Compares rewards of each task in the final EB and the terminal STE rewards for each task and measures how well the agent performs on all tasks after completing the syllabi: $T$ only includes the final EB, and $S(t)$ contains all tasks seen in the syllabus. \textbf{Relative reward after learning a task
% (RR\textsubscript{$\alpha$}):} Compares the rewards of the task learned in the preceding LB and the terminal STE reward for that task and measures how well the agent learns on the latest task averaged over the entire syllabus: $T$ includes all EBs, and $S(t)$ contains only the task learned in LB $t$. \textbf{Relative reward on known tasks (RR\textsubscript{$\sigma$}):} Compares rewards of all tasks that have appeared in prior LBs and the terminal STE rewards for those tasks and measures how well the agent performs on previously seen tasks (quantifies forgetting/ backward transfer): $T$ includes all EBs, and $S(t)$ contains all tasks in the syllabus encountered in previous LBs up to and including time $t$. % \textbf{Relative reward on unknown tasks (RR\textsubscript{$\upsilon$}):} Compares rewards of all tasks that have \textit{not} appeared in prior LBs and the terminal STE rewards for those tasks and measures how well the agent generalizes/transfers knowledge from seen to unseen tasks: $T$ includes all EBs, and $S(t)$ contains all tasks in the syllabus not encountered in previous LBs up to and including time $t$.

% \begin{itemize}
%     \item \textbf{Relative reward of the agent in the final EB (RR\textsubscript{$\Omega$}):} We compute the mean ratio between the mean rewards of each task in the final EB and the terminal STE rewards for each task. This measures how well the agent performs on all tasks after completing the syllabi. In this case, $T$ only includes the final evaluation block, and $S(t)$ contains all tasks seen in the syllabus.
%     \item \textbf{Relative reward of the agent after learning a task (RR\textsubscript{$\alpha$}):} We compute the mean ratio over all EBs between the mean reward of the task that was just learned in the previous LB and the terminal STE reward for that task. This measures how well the agent learns on the latest task averaged over the entire syllabus. In this case, $T$ includes all evaluation blocks, and $S(t)$ contains only the task learned in LB $t$.
%     \item \textbf{Relative reward of the agent on known tasks (RR\textsubscript{$\sigma$}):} We compute the mean ratio over all EBs between the mean rewards of all tasks that have appeared in prior LBs and the terminal STE rewards for those tasks. This measures how well the agent performs on previously seen tasks as a result of reducing forgetting and exhibiting backward transfer. In this case, $T$ includes all evaluation blocks, and $S(t)$ contains all tasks in the syllabus encountered in previous LBs up to and including time $t$.
%     \item \textbf{Relative reward of the agent on unknown tasks (RR\textsubscript{$\upsilon$}):} We compute the mean ratio over all EBs between the mean rewards of all tasks that have \textit{not} appeared in prior LBs and the terminal STE rewards for those tasks. This measures how well the agent generalizes/transfers knowledge from seen to unseen tasks. In this case, $T$ includes all evaluation blocks, and $S(t)$ contains all tasks in the syllabus not encountered in previous LBs up to and including time $t$.
% \end{itemize}

As mentioned, we employ established lifelong learning metrics defined by \citet{new2022lifelong}, which capture catastrophic forgetting, transfer between all pairs of tasks, and speed of learning. In all cases, more-positive values are better for all metrics. 
% We describe these metrics briefly and refer the reader to \citet{new2022lifelong} for details. 
\textbf{Forward Transfer Ratio (FTR)} is the ratio of EB performance on an unseen task. \textbf{Backward Transfer Ratio (BTR)} is the ratio of EB performance on a seen task. A value greater than one indicates positive transfer. \textbf{Relative Performance (RP)} is the ratio of the Area Under the Learning Curve (AUC) between the lifelong learner and STE learning curve. A value greater than one indicates either faster learning by the lifelong learner and/or superior asymptotic performance. \textbf{Performance Maintenance (PM)} is the average difference between task performance in any EB that comes after the LB of a seen task. 
%EB immediately after the last LB for that task. 
A value less than $0$ indicates forgetting. Refer to \citep{new2022lifelong} for more details about the metrics and the precise computation.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{graphics/alternating_curves.png}
\caption{Illustrative examples showing EB rewards of baseline and hidden replay in alternating tasks scenario. Column color denotes which task is trained in LBs between EBs. Left: Example syllabus of two similar tasks; the lifelong learner (LL) performs similarly to the baseline.
% , and some FT can be seen from the first to the second task. Middle and 
Right: Examples of two dissimilar tasks where the baseline exhibits catastrophic forgetting, our hidden replay does not.}
\label{fig:dissimilar_alternating}
\vspace{-0.75cm}
\end{figure}

\subsection{Domains} 

Our experiments use two RL domains: \SC{} minigames \citep{vinyals2017starcraft} and Minigrid \citep{gym_minigrid}. We evaluate on existing RL tasks (POMDPs) in these domains. 

\textbf{Starcraft 2}: 
%Our main testbed is built around SC-2 minigames following  \citep{vinyals2017starcraft}. 
We selected 3 minigames namely \emph{DefeatRoaches},  \emph{DefeatZerglingsAndBanelings}, and \emph{CollectMineralShards}. We created an additional task in each case as described in Appendix ~\ref{sec:sc2_task_descriptions}. We used PySC2 \citep{vinyals2017starcraft} to interface with SC-2 game. 
The agent receives positive rewards for collecting resources and defeating enemies, and negative rewards for losing friendly units. 
As observations, we used the unit type, selection status, and unit density two-dimensional inputs. 
% The action space is factored into functions and arguments, such as $\text{move}(x, y)$ or $\text{stop}()$. 
We follow the action space and convolutional policy network architecture defined in \citet{vinyals2017starcraft}. 
%, our policy networks output probabilities for the different action factors independently. 
Single task experts were trained to convergence ($\sim$ 30M environment steps using the VTrace algorithm \citep{espeholt2018impala}). We consider the pairwise, alternating, and condensed scenarios where each LB consists of 2 million environment steps (about 6\% of the STE samples), and each EB consists of 30 episodes per task. Complete details can be found in the Appendix \ref{sec:imp_sc2}.

\textbf{Minigrid}: 
Due to the heavy computational load of experimentation in SC-2, we also show results in the Minigrid domain \citep{gym_minigrid}. We use the TELLA framework \citep{lifelong-learning-systems} to orchestrate the experiments ($\sim$100 repetitions per scenario). Tasks involve an agent that must navigate to a goal while interacting with various entities in the environment. We consider 5 tasks --- SimpleCrossing, DistShift, a custom Fetch, a custom Unlock, and DoorKey --- each with two variants (differing in the size of the grid and/or number of objects) for a total of 10 POMDPs. Descriptions of these tasks can be found in \citet{gym_minigrid}. An observation is a $7\times7$ top-down view of the grid directly in front of the agent, with 3 channels containing information about the object type, object color, and object state in each tile. Rewards are sparse: $-1$ for running into obstacles and lava, $0$ for not reaching the goal, and a reward in $[0, 1]$ for reaching the goal proportional to the number of steps taken. There are only six actions: turn left, turn right, move forward, pick up an object, drop an object, and interact with an object. STEs are trained on each task for 1M environment steps using PPO \citep{schulman2017proximal}. We consider the pairwise and condensed scenarios where the LB lengths vary between 100k and 700k (Appendix~\ref{sec:minigrid_task_lengths}) based on examining the smallest number of steps for the STE to converge to $80\%$ of its peak performance averaged over ten runs. Each EB consists of 100 episodes per task. Further details can be found in Appendix~\ref{sec:imp_minigrid}.

\textbf{Baseline Agents}:
We compare against several non-lifelong baseline agents: 1) Random policy; 2) \emph{Baseline agent} using off-the-shelf deep RL trained on tasks in sequence without any lifelong learning. We used the VTrace algorithm \citep{espeholt2018impala} for SC-2 and PPO  \citep{schulman2017proximal} for the Minigrid experiments. 

\textbf{Ablations}: In order to compare different replay type, we perform ablations against the combination of buffers used for replay (see Fig. \ref{fig:all_replay_archs}): 1) \emph{Hidden Replay (ER)}, 2) \emph{Hidden Replay (ER+RaR)}, 3) \emph{Hidden Replay (ER+GR)}, 4) \emph{Hidden Replay (ER+RaR+GR)}. In each case, the VAE, sleep policy, and wake policy are trained, but on different augmented datasets as shown in Alg.~\ref{alg:hidden_replay} (samples are drawn from VAE only if GR is enabled).
Similarly, we perform ablations along architectures discussed in Fig.~\ref{fig:all_replay_archs}.

\textbf{Single Task Experiments}: 
%\textbf{Sleep Imitating Single Task Expert (STE)}: 
We conducted experiments that demonstrated that the wake-sleep training phases successfully imitates the STE. These can be found in the Appendix \ref{sec:ste_additional_results} for SC-2 and Minigrid. 
% We: i) Train an STE on each task/variant. ii)  Measure the final reward for each STE. iii) Load the trained STE and build a buffer of trajectories. iv) Train the sleep model until convergence on randomly sampled batches of observation-action pairs. v) Periodically evaluate the sleep model.
%  The two-headed and hidden replay architectures typically match or exceed the STE performance in terms of rewards. The sequential model learns non-trivial policies, but generally performs worse than the STE, supporting our hypothesis that decoupling the generator from the policy network results in better-performing policies. In Minigrid, we find that the average difference in rewards between the STE and hidden replay model's sleep policy's performance over all POMDPs is 0.14 with a standard deviation of 0.11, suggesting that the sleep policy is capable of imitating the STE to a high degree of precision.

\subsection{Evidence of Overcoming Catastrophic Forgetting}
We observed that different syllabi and scenarios can exhibit different levels of catastrophic forgetting due to varying degrees of similarity between the tasks in the syllabus. We first illustrate this issue before showing large scale results averaging over all syllabi.\footnote{We attempt to quantify pairwise similarity between tasks in Appendix \ref{sec:imp_sc2} by evaluating the forward transfer of the STE for each task to all other tasks. Quantifying task similarity remains an open problem.}
% We looked at how our proposed methods compares with the baseline (non-LL)  agent on syllabi involving transitioning between pairs of similar tasks vs pairs of dissimilar tasks.  
In Figure \ref{fig:dissimilar_alternating}, we illustrate examples that 
%the benefits of the proposed hidden replay model by looking at an example cases where 
1) the LL agent and non-LL agent perform similarly when syllabi are composed of similar tasks, and both agents exhibit positive FT and BT, and 2) the non-LL agent experiences catastrophic forgetting (zig-zag pattern) of one or both tasks whereas the LL agent shows significantly less forgetting \emph{when transitioning between two dissimilar tasks}. 
We note that in the \SC{} domain, evidence of extreme catastrophic forgetting is somewhat rare, a possible weakness in the design of our task set. Nevertheless, LL agents clearly outperform non-LL on almost all the other  metrics, signifying the need to look beyond catastrophic forgetting when evaluating LL. 
% a possible weakness in the design of our task set. We select several cases where forgetting is evident when transitioning between dissimilar tasks when using the baseline model, but this forgetting is averted when using the lifelong learning agent. 
% To better evaluate the strengths of the proposed model, we look at a series of quantitative metrics, including evaluating absolute performance against a single task expert (STE), as this is a more interpretable and relevant metric to real world applications. In the following section Doesn't seem to flow from the text

\subsection{Comparison of Different Types of Replay for Sleep}
\begin{figure*}[t]
\centering
\includegraphics[width=.98\textwidth]{graphics/minigrid_replay.png}
  \caption{Evaluating different replay types on the hidden replay model for the Minigrid domain. Error bars denote 95\% confidence interval.}
  \label{fig:minigrid_replay_ablations_main}
\end{figure*}

% \begin{figure*}[t]
% \centering
%     \includegraphics[width=0.24\textwidth, keepaspectratio]{graphics/Minigrid_Replay_Pairwise_LL.png}
%     \includegraphics[width=0.24\textwidth, keepaspectratio]{graphics/Minigrid_Replay_Condensed_PM.png}
%     \includegraphics[width=0.24\textwidth, keepaspectratio]{graphics/Minigrid_Replay_Condensed_LL.png}
%     \includegraphics[width=0.24\textwidth, keepaspectratio]{graphics/Minigrid_Replay_Condensed_RR.png}
%   \caption{Evaluating different combinations of replay types on the hidden replay model for the Minigrid domain}
%   \vspace{-15pt}
%   \label{fig:minigrid_replay_ablations_main}
% \end{figure*}

\begin{figure*}[t]
\centering
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Pairwise_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Alternating_PM.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Alternating_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Alternating_RR.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Condensed_PM.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Condensed_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Replay_Condensed_RR.png}
    \includegraphics[width=0.98\textwidth]{graphics/sc2_replay.png}
  \caption{Evaluating different replay types on the hidden replay model for the \SC{} domain. Error bars denote 95\% confidence interval.}
  \label{fig:sc2_replay_ablations_main}
\end{figure*}

To understand the effect of different replay types on the hidden replay model: experience replay from the wake buffer (ER), generative replay (GR), and random replay (RaR). All approaches still train both the policy network and generator, even if GR is disabled. We summarize the important findings in Fig.~\ref{fig:minigrid_replay_ablations_main} and Fig.~\ref{fig:sc2_replay_ablations_main} \footnote{Further experiments can be found in Appendix \ref{app:replay_ablation}}.

\textbf{Transfer Learning and Generalization to Unseen Tasks}: 
Looking at the pairwise scenario in Minigrid and \SC{}, we see that models that use hidden replay with ER+GR, ER+RaR or ER+RaR+GR show much higher FT compared to the baseline. Hidden replay with ER+GR, ER+RaR or ER+RaR+GR show higher $RR_\upsilon$ and the effect is more pronounced for \SC{}  condensed scenario, showing generalization to unseen tasks. 
% , we see that the models that use RaR generalize well to unknown tasks. 

\textbf{Mitigating Catastrophic Forgetting}:
Looking at PM across all scenarios in Minigrid and \SC{} and looking at  $RR_\Omega$ of the Minigrid condensed scenario, we validate that the hidden replay model requires stabilization with RaR in order to (significantly) reduce catastrophic forgetting, compared to ER+GR alone which is typically worse than ER+RaR and ER+RaR+GR.

\textbf{Adaptation to New Tasks}: Interestingly, we find that $RR_\alpha$ for the condensed scenarios of Minigrid and \SC{}, shows that simply performing distillation during sleep phases produces 
% seems to help prevent interference and possibly introduce 
a beneficial ``jumpstart'' effect when learning new tasks, compared to the baseline which is also able to learn the new task but requires more learning experiences. 

\textbf{Backward Transfer}: The BT metric seems to vary across the board based on the type of replay used. This is in part because when computing the BT metric from task 2 to task 1, it is very sensitive to how well the model learns on task 1. If the model learns task 1 to near optimal performance, it is very difficult to achieve $BT>1$ whereas if task 1 is not well-learned, even a weak model on a similar task 2 can potentially easily achieve $BT>1$. However, if we look at $RR_\sigma$ instead, we see a different story where the models that learn best (ER+RaR and ER+RaR+GR) often exhibit the best performance on seen tasks in opposition to the BT metric.

\textbf{General Observations}: 
% already talked about this in above
% We observe that standard generative hidden replay (ER + GR) can hurt performance. 
Adding a small amount of random replay (ER+RaR+GR) fixes many issues with standard generative hidden replay, producing noticeably better results. We find that ER+RaR, even without GR, achieves significant improvement over the baseline agent, and the model further improves when all types of replay (ER+RaR+GR) are combined, albeit by a small amount. This suggests that RaR of a small number of samples is often powerful and 
% GR interacts with ER + RaR in a 
complementary (i.e., often helpful, rarely hurtful) to GR (n.b.\! all methods train the VAE, but only GR samples from it). This leads us to suspect that the replay architecture is more important than the sampling strategy that we investigate next. 
% but limited way. 
% This highlights a weakness in our evaluation methodology, suggesting that the tasks we selected might require relatively simple and consistent policies that do not require the use of more complex GR.

% \textbf{General Observations}: We observe that standard generative hidden replay (ER + GR) can hurt performance in terms of the metrics. However, adding a small amount of random replay (ER + RaR + GR) instead produces noticeably better results. We find that ER + RaR in general often achieves significant improvement over the baseline agent in terms of the aforementioned properties, and the model further improves when all three types of replay (ER + RaR + GR) are combined. This suggests that random replay of a small number of samples is often very powerful and generative replay interacts with ER + RaR in a complementary (i.e., often helpful, rarely hurtful) but limited way. This also highlights a weakness in our evaluation methodology, suggesting that the tasks we selected might require relatively simple and consistent policies that do not require the use of the more complex generative replay.

\subsection{Comparison of Different Architectures for Sleep}
% \begin{figure*}[t]
% \centering
%     \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/Minigrid_Archs_Pairwise_LL.png}
%     \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/Minigrid_Archs_Condensed_PM.png}
%     \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/Minigrid_Archs_Condensed_LL.png}
%     \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/Minigrid_Archs_Condensed_RR.png}
%   \caption{Evaluating the performance of different architectures for the Minigrid domain.}
%   \label{fig:minigrid_system_ablations_main}
%   \vspace{-0.5cm}
% \end{figure*}

\begin{figure*}[t]
\centering
    \includegraphics[width=0.98\textwidth]{graphics/minigrid_archs.png}
  \caption{Evaluating the performance of different architectures for the Minigrid domain. Error bars denote 95\% confidence interval.}
  \label{fig:minigrid_ablations_archs_main}
\end{figure*}

\begin{figure*}[t]
\centering
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Pairwise_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Alternating_PM.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Alternating_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Alternating_RR.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Condensed_PM.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Condensed_LL.png}
    % \includegraphics[width=0.22\textwidth, keepaspectratio]{graphics/SC2_Archs_Condensed_RR.png}
    \includegraphics[width=0.98\textwidth]{graphics/sc2_archs.png}
  \caption{Evaluating the performance of different architectures for the \SC{} domain. Error bars denote 95\% confidence interval.}
  \label{fig:sc2_ablations_archs_main}
  \vspace{-0.5cm}
\end{figure*}

We aim to understand the strengths and weaknesses of the model architectures introduced in this paper (Sequential, Two-Headed, Hidden Replay) and understand how these models improve over simple baselines. 
% (random agent, baseline RL agent, distillation-only agent) in lifelong learning settings. 
We summarize the important findings in Fig.~\ref{fig:minigrid_ablations_archs_main} and Fig.~\ref{fig:sc2_ablations_archs_main} \footnote{Further experiments can be found in Appendix \ref{app:archs_ablation})}.

\textbf{Transfer Learning and Generalization to Unseen Tasks}: Forward transfer seems to be a strength of the hidden replay model.  Looking at FT across all domains and scenarios and looking at the $RR_\upsilon$ of the \SC{} scenarios, we see that the hidden replay model noticeably outperforms the other models.

\textbf{Avoiding Catastrophic Forgetting}:
Looking at PM and $RR_\Omega$ across all scenarios, the hidden replay model often outperforms the other models.

\textbf{Adaptation to New Tasks}: We see that the hidden replay model achieves consistently high (and often the best) RP and $RR_\alpha$ across most scenarios in both domains. This suggests that the hidden replay model is not interfering with new tasks and may be providing a helpful ``jumpstart'' effect. 

\textbf{Positive Backward Transfer}: As before, it can be difficult to interpret the BT metric. In general, the BT of the hidden replay model is on par with other models that achieve comparable terminal performance, and the hidden replay model shows strong performance in terms of $RR_\sigma$.

\textbf{Sample Efficiency}
Compared to STE, our experiments using the hidden replay model required only 6\% of training samples to achieve 80-90\% of expert performance in most \SC{} scenarios.

\textbf{General Observations}: In general, across both domains and many scenarios, the hidden replay model seems to outperform the other model architectures tested in most of the metrics of interest. This suggests that the hidden replay model is a potentially powerful model for addressing lifelong RL. We observe (in the case of the Minigrid experiments where all types of replay are used for all architectures), architecture seems to play a more significant role in improving lifelong learning performance than the type of replay. 

==> SRI CoLLA 2022 L2M Paper Revised/introduction.tex <==
\section{Introduction}

%\note{TODO: Probably needs tighter connections to existing literature}

Lifelong Reinforcement Learning (LRL) involves training an agent to maximize its cumulative performance on a stream of changing \textit{tasks} over a long lifetime. LRL agents must balance \textit{plasticity vs. stability}: learning the current task while maintaining performance on previous tasks. Deep neural networks are especially prone to instability, often exhibiting \textit{catastrophic forgetting} of previous tasks when trained on multiple tasks that are presented sequentially  \citep{kirkpatrick_overcoming_2016}. One approach to meet the challenges of deep LRL is by careful managing the agent's learning experiences, in order to learn (without forgetting) and build internal meta-models (of the tasks, environments, agents, and world). One strategy for managing experiences is to recall data from previous tasks and mix it with data from the current task when training, essentially transforming sequential LRL into batch multi-task reinforcement learning (RL) \citep{brunskill2013sample}. The technique of \textit{experience replay} of past data is common in deep RL \citep[e.g.][]{mnih2013playing} and has been studied in the lifelong learning literature \citep{isele2018selective,rolnick2019experience,hayes2021replay}. 
However, storing sufficient examples from all previous tasks may be unreasonable in systems with limited resources or long lifetimes.
Rather than store an ever-growing list of experiences, one can instead employ \textit{generative replay} (GR) \citep{shin2017continual,van_de_ven_generative_2018}, a biologically-inspired replay mechanism that augments learning experiences with self-labelled examples drawn from an internal generative model trained to approximate the distribution of past experiences. 
% In general, the data distribution $p(x,y)$ is factored as $p(y|x)p(x)$, where $p(x)$ is learned by a generative model and $p(y|x)$ is learned by a discriminative model.
%or \emph{skill} that predicts an output $y$ for input $x$ (i.e., a classifier in supervised learning or a policy in reinforcement learning).

% In this work, we study agent architectures for LRL that use GR for memory consolidation in \emph{wake-sleep} phases. 
In LRL (see \citet{khetarpal2020towards} for a survey), each task is a Markov decision process (MDP), and the agent must learn a policy for interacting with its environment to maximize its lifetime performance (e.g., average reward over all tasks). 
While GR has been shown to be effective in lifelong supervised learning \citep{van_de_ven_generative_2018}, it has been less explored in LRL. 
The LRL setting is complicated by the fact that the agent's experiences are observation-action \emph{trajectories} whose distribution depends on the environment dynamics and the policy being executed. 
While prior work with world models \citep{ketz2019continual} and pseudo-rehearsal \citep{atkinson2021pseudo} focused on generative replay of (partial) trajectories, this requires modeling the dynamics, which is difficult in complex environments. 
% In contrast, most popular current deep RL algorithms are \emph{model-free} and do not learn the dynamics explicitly.

In this paper, we present agent architectures for LRL that use GR for memory consolidation and 
% a version of generative replay for LRL that satisfies 
satisfy two desiderata: (a) Introspective density modelling of the latent representations of policies learned using deep RL, and (b) Model-free end-to-end learning. 
The first property avoids the challenges of density modelling of complex high-dimensional perceptual inputs, whereas policy learning using deep RL works well with such perceptual inputs. 
The second property avoids the challenges of learning temporal dynamics and reward functions from few learning experiences with sparse rewards. 
Our contributions extend powerful \emph{model-free} deep RL and do not learn the dynamics explicitly.

Our first contribution is a model-free approach to generative replay (Section \ref{sec:model-free-generative-replay}) in lifelong RL. We empirically demonstrate that replay of independently sampled observation-action pairs is sufficient to mitigate forgetting. This is noteworthy because observation-action pairs are simpler to generate than trajectories, and because replay of observation-action pairs is directly analogous to replay of input-label pairs in supervised learning, thus unifying generative replay methods for lifelong learning.

Our second contribution is a mechanism for memory consolidation via \emph{wake-sleep} cycles. During \emph{wake phases}, our agent improves a policy for the current task(s) using an off-the-shelf RL algorithm while storing samples of experiences in a buffer. Periodically, the agent enters a \emph{sleep phase}, during which the generative memory is trained to model the agent's new experiences, and the procedural knowledge embodied in the policy learned during the wake phase is consolidated into the agent's ``skill set'' via policy distillation \citep{rusu2015policy} with GR. In the next wake phase, a new exploration policy is seeded with knowledge from previously-learned skills, and the cycle repeats. 
% We show that this wake-sleep mechanism prevents forgetting while facilitating forward transfer to novel tasks.
%There are many possible instantiations of model-free generative replay. 
We investigate three different replay architectures (Section \ref{sec:model-free-generative-replay}) within the wake-sleep framework, starting from a na\"ive generative and adding ingredients to achieve the aforementioned introspective density modelling of the latent representations and model-free end-to-end learning.

We evaluate our algorithm and architectural contributions through experiments (Section \ref{sec:experiments}) on three different scenarios comprising tasks from the \SC{} (SC-2) and Minigrid domains. We report several key findings showing the impact of the design choices on quantitative metrics that include transfer learning, generalization to unseen tasks, fast adaptation after task change, performance compared to  task experts, and catastrophic forgetting.   
We observe that our GR prevents drift in the features-to-action mapping of a deep RL agent (that learns the features from observations). We find that \emph{hidden replay} (replay of such features) outperforms other replay mechanisms, which agrees with past results in lifelong supervised learning \citep{van2020brain}. Since deep RL in SC-2 is computationally demanding, we release a dataset of trajectories of trained single-task expert policies for future research \footnote{\url{https://github.com/sri-l2m/l2m\_data}}.

% Our comprehensive results show improved performance over na\"{i}ve RL agents in terms of established quantitative metrics for lifelong learning \citep{new2022lifelong}. 

%There are many open questions in applying generative memory to the task of lifelong reinforcement learning including:
%\begin{itemize}
%    \item Does generative replay for reinforcement learning require the replay of entire trajectories (i.e., a ``model-based'' approach towards generative replay) or is replaying random, independent state-action pairs (i.e., a ``model-free'' approach towards generative replay) sufficient?
%    \item Must replayed trajectories/transitions be on-policy and on-task, or can they be arbitrarily sampled from previous policies and tasks? 
%\end{itemize}

%Past work in world models \citep{ketz2019continual} and pseudo-rehearsal \citep{atkinson2021pseudo} show generating entire or partial trajectories is sufficient towards achieving lifelong learning. This work considers the setting where independent state-action pairs are replayed and under such a setting, improvement is shown with respect to lifelong learning metrics compared to non-lifelong learning agents. Furthermore, this work demonstrates that using model-free generative memory that generates off-policy and off-task samples still exhibits improvement in terms of lifelong learning metrics compared to non-lifelong learning agents. Our findings have significant impact because state-action pairs are simpler to generate than entire trajectories and replaying state-action pairs helps to unify lifelong reinforcement learning with lifelong supervised learning (i.e., state-action pairs are analogous to observation-label pairs). This observation leads us to developing a novel method for training lifelong RL agents via a wake-sleep mechanism. We show that model-free generative replay can operate in a task-agnostic manner in ``wake-sleep'' phases, where sleep phase learns to consolidate policies for past tasks with a policy for the current task using a novel combination of generative replay and policy distillation, and the wake phase uses the consolidated sleep policy for off-policy learning and exploration of the current task. We empirically demonstrate that single task learning using wake-sleep phases converges to near-optimal policies and wake-sleep models achieve improved performance in lifelong learning settings in terms of catastrophic forgetting and transfer. 

% \sout{Our third contribution, and a distinguishing aspect of this work, is an integration of our core framework of wake-sleep and  model-free generative replay with multiple independently-developed components (Section \ref{sec:integration}) that address different aspects of the lifelong learning problem. Our multi-institution team developed a component-based architecture that allows for fair comparison of different combinations of components within a common evaluation environment. We experimentally validate that integrating the following components results in improved lifelong learning metrics and system capabilities: mixture modeling of disparate tasks using multiple generative models; sleep phases triggered adaptively via continual changepoint detection; compression of experiences using quantization; prioritized replay using continual danger detection; and representation learning via unsupervised and self-supervised learning.}

%The wake-sleep mechanism and model-free generative replay are flexible frameworks and can be easily extended to handle more complex use cases via integration with other lifelong learning components. We integrate recently published continual learning algorithms within the context of wake-sleep phases in order to overcome some of the limitations of the wake-sleep mechanism. 
%We experimentally validate that integrating the following components results in improved lifelong RL via improved lifelong learning metrics and/or system capabilities: mixture modelling of disparate tasks using multiple generative models, sleep phase triggered in an adaptive manner using continual changepoint detection, compression of experiences using continual tensor quantization, prioritized replay using continual danger detection, and learning novel representations of input observations via unsupervised and self-supervised learning.

% \sout{, and demonstrate the viability of integrated lifelong learning systems composed of heterogeneous components.}

% In the face of task changes, these work by interleaving experience across tasks thereby interleaving updates and stabilizing learning of new tasks with avoiding forgetting of old tasks.
% The technical contributions of this paper include the following:
% \begin{itemize}
%     \item We explore generative replay in the context of lifelong reinforcement learning settings.
%     \item We show that generative replay is able to work on individual (state, action) pairs, which is in contrast to previous literature which replayed entire trajectories. This unifies lifelong reinforcement learning with lifelong supervised learning.
%     \item We examine iterative policy distillation where an RL agent learns to mimic off-policy and off-task (state, action) pairs generated by a different agent. 
%     \item We show how iterative policy distillation can be used in a wake-sleep cycle-based learning procedure where a wake agent learns a policy for a single task, and the sleep agent periodically consolidates the wake agent's policy with previous policies (from previous tasks and non-stationary wake agents on the same task).
%     \item We show that the benefit of generative replay for RL can be higher with careful choice of architecture and combination of different replay mechanisms. We explore three different architectures for our sleep agent, which each utilize generative replay in different ways: sequential, two-headed, and hidden replay.
%     \item We show how generative replay can be extended in several ways: learning mixtures of generative models using Eigentasks, identifying when to consolidate knowledge via changepoint detection, compressing the wake replay buffer data, learning unsupervised and self-supervised representations of the observation space, and a domain-specific use-case: detecting and avoiding dangerous states.
%     \item We demonstrate and validate our approach using minigames from the real-time strategy game StarCraft-2 as well as using a simpler grid-world setting: Minigrid.
%     \item We release data for exploring lifelong learning in the StarCraft-2 setting.
% \end{itemize}


%The technical contributions of this paper include the following:
%\begin{itemize}
%    \item We formulate, investigate, and validate the Eigentask framework for lifelong supervised and reinforcement learning problems.
    %\item We investigate combining knowledge distillation with off-policy reinforcement learning via iterative policy distillation.
    %\item We experimentally validate that iterative policy distillation works in sequential task settings.
    %\item We develop a complete system based on the Eigentask framework that can be used for learning to play real-time strategy games and release code and data for exploring lifelong learning in the StarCraftII setting.
    %\item We demonstrate that the Eigentask framework can be combined with other machine learning and lifelong learning methods in order to extend the framework's capabilities for more complex settings.
%\end{itemize}

==> SRI CoLLA 2022 L2M Paper Revised/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> SRI CoLLA 2022 L2M Paper Revised/setup.tex <==
\section{Background}
\subsection{Lifelong Reinforcement Learning (LRL) Setup}

% A lifelong RL \emph{syllabus} is a sequence of \emph{tasks} that the learning agent experiences one at a time for a fixed number of interactions. Each task is assumed to be formulated as a Markov Decision Process (MDP) \cite{sutton2018reinforcement}. 
% An MDP is a tuple $(\States, \Actions, P, R)$, where $\States$ is a finite set of states, $\Actions$ is a finite set of actions, $P : \States \times \Actions \mapsto \Prob(\States)$ is the transition function, $R : \States \times \Actions \mapsto \Reals$ is the reward function. %, $P_0$ is the distribution of initial states, and $\gamma \in (0, 1]$ is the discount factor. 
% The objective is a policy $\pi : \States \mapsto \Prob(\Actions)$ that maximizes the value function $V^{\pi}(s) = E_{S_t \sim P, A_t \sim \pi}[\sum_{t = 1}^{\infty} \gamma^t R(S_t, A_t)]$. Tasks in lifelong RL are MDPs, with common state and action spaces, but $P$ and $R$ may differ. % The input space $\mathcal{X}$ is the set of states $\States$, the output space $\mathcal{Y}$ is the set of actions $\Actions$, and 
% The loss is the negative return, $L(\mathbf{x}, \mathbf{y}) = -\sum_{(x, y) \in (\mathbf{x}, \mathbf{y})} R(x, y)$. % The input distribution is the distribution of state trajectories induced by the agent's behavior policy.
% %A rigorous definition of task that encompasses both supervised learning and RL would significantly complicate the notation, but we will %manage with the intuitive notion that task $=$ MDP for the purposes of this paper.

A lifelong RL \emph{syllabus} is a sequence of \emph{tasks} that the learning agent experiences one at a time for a fixed number of interactions.
Each task is assumed to be formulated as a Partially Observable Markov Decision Processes (POMDPs) \citep{sutton2018reinforcement}, where 
% POMDPs are generalizations of Markov Decision Processes where the agent cannot observe the state of the system directly. 
each POMDP is defined by a tuple $(\mathcal{S}, \mathcal{A}, P(s'|s,a), R(s, a), \mathcal{O}, Z(o|s))$ consisting of set of states $\mathcal{S}$, a set of actions $\mathcal{A}$, a transition probability function between states $P(s'|s,a)$, a reward function $R(s, a)$, a set of observations $\mathcal{O}$, and conditional observation probability function $Z(o|s)$.

We assume that all tasks have distinct observation spaces of the same dimensionality, share a common action space (e.g., point-and-click, issue movement or attack commands), but differ in the transition and reward dynamics.
For example, this setup can capture the use case of an embodied agent using the same set of sensors and actuators throughout their lifetime but with different reward functions or objectives. 

In single-task RL, the objective is to learn a policy that maps the history of observations to actions, $\pi: \mathcal{O}^h \rightarrow \mathcal{A}$, such that the policy maximizes the expected discounted future reward, given by the value function $V^{\pi}(s) = E_{S_t \sim P, A_t \sim \pi}[\sum_{t = 1}^{\infty} \gamma^{t-1} R(S_t, A_t)]$. We will refer to the task-optimal policy as a \emph{single task expert} (STE).

 

%\note{replay buffer should be introduced here; Z: Not sure I agree, this section is introducing the overarching problem of Lifelong RL; replay is a solution to that problem, but not part of the problem itself}

%Lifelong Learning involves training an agent to continually learn from a stream of \textit{tasks} over long lifetimes. As the agent encounters new tasks, it must accumulate and leverage knowledge to learn novel tasks faster (positive forward transfer), while maintaining performance on previous tasks (minimizing catastrophic forgetting or negative backwards transfer). In this paper, we consider the task of lifelong reinforcement learning. Our tasks are defined as Partially Observable Markov Decision Processes (POMDPs). POMDPs are generalizations of Markov Decision Processes where the dynamics of a system are governed by an MDP, but an agent is unable to directly observe the state of the system. POMDPs are defined by a tuple $(S, A, P(s_{j}|s_{i},a), R(s, a), O, P(o|s))$ consisting of set of states $s_{0}, ..., s_{n}  \in S$, a set of actions $a_{0}, ..., a_{m}  \in A$, a probabilistic transition function between states $P(s_{j}|s_{i},a)$, a reward function mapping states and actions to a reward $R(s, a)$, a set of observations $o_{0}, ..., o_{l} \in O$, and a set of conditional observation probabilities $P(o|s)$. In standard RL (i.e., for a single task) the goal is to learn a policy that maps observations to actions $\pi: O \mapsto A$ by maximizing the value function $V^{\pi}(s) = E_{S_t \sim P, A_t \sim \pi}[\sum_{t = 1}^{\infty} \gamma^t R(S_t, A_t)]$ the expected discounted (by $\gamma$) cumulative rewards over an entire episode (from initial state to terminal state). When an RL agent is deployed, it receives an observation from the current state of the environment, and selects and takes the action based on the policy to transition to the next state.


% \note{More explanation needed on shared obs action spaces}
Lifelong Learning involves training an agent to continually learn from a stream of tasks over long lifetimes. 
As the agent encounters new tasks, it must accumulate and leverage knowledge to learn novel tasks faster (positive forward transfer), while maintaining performance on previous tasks (minimizing catastrophic forgetting or negative backwards transfer).
In this paper, we consider the task of lifelong reinforcement learning (LRL), which has been less explored than class-incremental classification \citet{hayes2021replay} in the literature.

% Our tasks are defined as Partially Observable Markov Decision Processes (POMDPs). POMDPs are generalizations of Markov Decision Processes where the dynamics of a system are governed by an MDP, but an agent is unable to directly observe the state of the system. POMDPs are defined by a tuple $(S, A, P(s_{j}|s_{i},a), R(s, a), O, P(o|s))$ consisting of set of states $s_{0}, ..., s_{n}  \in S$, a set of actions $a_{0}, ..., a_{m}  \in A$, a probabilistic transition function between states $P(s_{j}|s_{i},a)$, a reward function mapping states and actions to a reward $R(s, a)$, a set of observations $o_{0}, ..., o_{l} \in O$, and a set of conditional observation probabilities $P(o|s)$. In standard RL (i.e., for a single task) the goal is to learn a policy that maps observations to actions $\pi: O \mapsto A$ by maximizing the value function $V^{\pi}(s) = E_{S_t \sim P, A_t \sim \pi}[\sum_{t = 1}^{\infty} \gamma^t R(S_t, A_t)]$ the expected discounted (by $\gamma$) cumulative rewards over an entire episode (from initial state to terminal state). When an RL agent is deployed, it receives an observation from the current state of the environment, and selects and takes the action based on the policy to transition to the next state.

The objective in LRL is to learn a policy that maximizes average cumulative reward over all POMDPs in a task set while learning from limited interactions with a sequence of POMDPs drawn from the task set.
This is challenging because the learning problem is non-stationary and the learner needs to accommodate an increasing number of tasks in a model with fixed capacity.
The task changes after an unknown number of interactions with the environment. 
The agent has no control over the choice of the next task. 
In our setting the agent has no knowledge of the identity of the current task, or the transition points between tasks.
% In addition to tasks, we introduce  \emph{variants} of each task. All variants of a task are conceptually similar (e.g., different formations of enemy units in SC-2). 

%In the case that two tasks are qualitatively similar in terms of the agents' goal but differ in one or more significant task parameters, we refer to them as ``variants'' of the same tasks. For example, our SC2 task set consists of a total of three tasks and two variants per task for a total of six different MDPs, where one task might be defeating a specific type of enemy and its variants entail different numbers or starting positions of units. 

% In Fig. \ref{fig:sc2_learning_curves}, we show an example of an agent that is capable of learning across a lifetime of six task variants while achieving performance comparable to single-task experts on each task and exhibiting some forward transfer and reduced forgetting.

% \begin{figure*}[t]
% \begin{minipage}{0.53\textwidth}
% \centering
%     \includegraphics[width=0.95\textwidth, keepaspectratio]{graphics/scenarios.png}
%   \caption{Lifelong Learning Scenarios. Grey evaluation blocks (EBs) evaluate the agent on all tasks. Learning blocks (LBs) are color coded by task, and subscripts denote task variants.}
%   \label{fig:scenarios}
% \end{minipage}
% \hfill
% \begin{minipage}{0.43\textwidth}
% \centering
%     \includegraphics[width=0.9\textwidth, keepaspectratio]{graphics/metrics.png}
%   \vspace{-0.2cm}
%   \caption{Illustration of FTR and BTR metrics \cite{new2022lifelong}.}
%   \label{fig:metrics}
% \end{minipage}
% \end{figure*}

% \subsection{Scenarios}
% \label{sec:scenarios}
% %\begin{wrapfigure}{r}{0.45\textwidth}
% %\centering
% %    \includegraphics[width=0.35\textwidth]{graphics/scenarios.png}
% %  \caption{Lifelong Learning Scenarios. Grey evaluation blocks (EB) evaluate the agent on all tasks. Learning blocks are color coded by task, and subscripts denote task variants.}
% %  \label{fig:scenarios}
% %\end{wrapfigure}
% A lifelong learning \textit{scenario} describes the order of task presentation and repetition of tasks and corresponds to a set of syllabi. The four kinds of scenarios are depicted in Figure~\ref{fig:scenarios}. Each scenario alternates between \emph{evaluation blocks} (EBs) and \emph{learning blocks} (LBs) \citep[see][]{new2022lifelong}. We say that a task (variant) is \emph{known} if it has appeared in an LB; otherwise it is \emph{unknown}. During each EB, the agent is evaluated on all task variants in the scenario (including unknown tasks); during each LB, the agent learns on a single task variant. 
% \textbf{Single Task:} This serves as a baseline and measures the optimal performance of a learner on a task. \textbf{Pairwise:} Two tasks are presented once each. This scenario evaluates knowledge transfer between two tasks. \textbf{Alternating:} Two tasks are presented with three repetitions of each pair. This scenario evaluates knowledge retention over longer lifetimes. \textbf{Condensed:} A random permutation of all tasks is presented. Task variants appear after all tasks have been seen once. This is a useful setting for understanding how an agent performs across different task orderings. \textbf{Dispersed:} A task sequence from a Condensed scenario is repeated multiple times. In our experiments, we repeat a Condensed scenario three times, but with LBs of one-third the size. The dispersed scenario evaluates knowledge accumulation in the face of rapid task changes where experience is dispersed over time.

% %\begin{description}
% %\item[\textbf{Single Task: }] This serves as a baseline and measures the optimal performance of a learner on a task. 
% %\item[\textbf{Pairwise: }] Two tasks are presented once each. In each task, the agent experiences a fixed number of learning steps.  This scenario evaluates knowledge transfer between two tasks. 
% %\item[\textbf{Alternating: }] Two tasks are presented with three repetitions of each pair. This scenario evaluates knowledge retention in longer lifetimes.
% %\item[\textbf{Condensed: }] A random permutation of all tasks is presented. Task variants do not appear again until all tasks have been encountered at least once. This is a useful setting for understanding how an agent performs across different orderings of tasks. 
% %\item[\textbf{Dispersed: }] This scenario repeats a task sequence from the condensed scenario multiple times. In our experiments, we repeat a condensed scenario three times, but the learning blocks are reduced to one-third the size. This scenario evaluates knowledge accumulation in the face of rapid task changes where experience is dispersed across time.
% %\end{description}

% % \ref{sec:scenarios_app} of the Appendix:

% %\begin{itemize}
% %    \item \textbf{Single Task: } This serves as a baseline and measures the optimal performance %of a learner on a task.
% %    \item \textbf{Pairwise: } Two tasks are presented one after the other. In each task, the %agent experiences a fixed number of learning steps.  This scenario evaluates knowledge transfer %between two tasks.
% %    \item \textbf{Alternating: } Two tasks are presented with three repetitions of each pair. %This scenario evaluates knowledge retention in longer lifetimes.
% %    \item \textbf{Condensed: } A random permutation of all tasks is presented. Task variants do %not appear again until all tasks have been encountered at least once. This is a useful setting %for understanding how an agent performs across different orderings of tasks.
% %    \item \textbf{Dispersed: } This scenario repeats a task sequence from the condensed scenario %multiple times. In our experiments, we repeat a condensed scenario three times, but the learning %blocks are reduced to one-third the size. This scenario evaluates knowledge accumulation in the %face of rapid task changes where experience is dispersed across time.
% %\end{itemize}

% % \subsection{Scenarios for Evaluating Lifelong Learning Agents}
% % \label{sec:scenarios_app}
% % \begin{figure}[H]
% % \centering
% % \includegraphics[width=0.95\textwidth]{graphics/scenarios.png}
% % \caption{Visualizations of the different scenarios tested.}
% % \label{fig:scenarios}
% %\end{figure}

% \subsection{Metrics for Lifelong RL}
% %\begin{wrapfigure}{r}{0.40\textwidth}
% %\centering
% %    \includegraphics[width=0.35\textwidth]{graphics/metrics.png}
% %  \caption{Illustration of FTR and BTR metrics.}
% %  \label{fig:metrics}
% %\end{wrapfigure}
% We employ the lifelong learning metrics defined by \citet{new2022lifelong}. More-positive values are better for all metrics.
% %In contrast to the ``Continuous RL'' setup \citep{normandin2021sequoia}, 
% %At the start of the lifetime and after every learning block, an evaluation blockThe lifelong learner is evaluated on every task (including unseen tasks) after each learning block and at the start of the lifetime. These are called evaluation blocks (EB) in  \cite{new2022lifelong}.
% \textbf{Forward Transfer Ratio (FTR)} is the ratio of EB performance on an \emph{unknown} task (see Figure \ref{fig:metrics}). \textbf{Backward Transfer Ratio (BTR)} is the ratio of EB performance on a known task. A value greater than one indicates positive transfer. \textbf{Relative Performance (RP)} is the ratio of the Area Under the Learning Curve (AUC) between the lifelong learner and a single task learner. A value greater than one indicates either faster learning by the lifelong learner and/or superior asymptotic performance. \textbf{Performance Maintenance (PM)} is the average difference between task performance in subsequent EBs compared to the EB immediately after the last LB for that task. A value less than $0$ indicates forgetting. Refer to \cite{new2022lifelong} for more details about the metrics and the precise computation.

% %\paragraph{CUT CANDIDATE} We choose these metrics over alternatives \citep[e.g.][]{normandin2021sequoia} because they apply to a broad range of lifelong learning settings (e.g., transfer to tasks not explicitly in the scenario, capturing impact of task repetitions, comparisons to non-lifelong learning agents, etc.) while still capturing important information about transfer and catastrophic forgetting in a standardized manner. Nevertheless, it should be noted that each metric is more or less useful in different scenarios --- for example, PM is more relevant in condensed scenarios as it accounts for all task changes that occur in long lifetimes, whereas BTR/FTR transfer metrics are more useful in pairwise scenarios.

\subsection{Generative Replay (GR)}
Our work is focused on generative replay (GR), which can be broadly described as a form of data augmentation where real-world experiences are used to continually train a generative model over the input space of the problem. Subsequently, data sampled from this generator can be pseudo-labeled or self-labeled to generate paired training examples that may reflect previously trained tasks. 
Different types of replay were discussed by \citet{hayes2021replay} along with its role in the brain and in current deep learning implementations. Most of the prior work on generative replay has focused on the problem of class-incremental classification \citet{van_de_ven_three_2019,shin2017continual}, or class-incremental generative modelling \citet{cong2020gan} as a subroutine thereof, but there has been significantly less exploration of GR in LRL.

We use a Variational Auto-Encoder (VAE) \citep{kingma_auto-encoding_2014} as the generative model. The VAE consists of an encoder $q_\phi(z|o)$ mapping observations to a vector-valued latent space $z$, and a decoder $p_\theta(o|z)$ that is trained to reconstruct the original input. We use the Gaussian prior $z \sim N(0, \mathbf{I})$ with 0 mean and unit variance $\mathbf{I}$. To train the VAE, we minimize the standard loss $\mathcal{L}_\text{VAE}$, 
\begin{equation}
\label{loss:vae}
\min E_{q_{\phi}(z|o)}[\ln p_{\theta}(o|z)] - D_{KL}[q_{\phi}(z|o)||p(z)]
\end{equation}
%Generative replay can balance stability on past tasks with plasticity on new tasks and mitigate catastrophic forgetting. 
% We seek a version of GR for LRL that satisfies two desiderata: (a) Introspective density modelling of the latent representations of policies learned using deep RL, and (b) Model-free end-to-end learning.
% The first property avoids the challenges of density modelling of complex high-dimensional perceptual inputs, whereas policy learning using deep RL works well with such perceptual inputs.
% The second property avoids the challenges of learning temporal dynamics and reward functions from few learning experiences with sparse rewards.
World models \citep{ketz2019continual} use model-based generative replay for LRL i.e., the replay generates rollouts or entire trajectories \citep[e.g.][]{ketz_using_2019}. Model-based replay works well in many domains, but it is challenging for domains such as SC-2 due to the complex dynamics and high dimensional observation and action spaces.
The most relevant prior work is that of \citeauthor{atkinson2021pseudo} \citep{atkinson2021pseudo} who explored model-free generative replay for Deep Q-Learning (DQN). 
However, \citet{atkinson2021pseudo} uses GANs in the raw perceptual space of the agent (aka veridical replay \citet{hayes2021replay}). Others have explored sophisticated strategies for prioritized experience replay in DQN  \citep[e.g.][]{isele2018selective, riemer2019scalable,wang2021acae,caccia2020online,zhang2017deeper,schaul2015prioritized} in LRL, but these are not generative in nature. 
We show that na\"ively migrating the generative modelling (similar to \citeauthor{atkinson2021pseudo}) to the feature space of the policy causes instabilities and severe catastrophic forgetting. 
% In the next section, we show that the issue is caused by drift in the feature extractor, and circumvent the issue by retaining an additional but small buffer of randomly selected experiences.
%need to say that model based approach seems hard for highly complex simulators like SC2
To the best of our knowledge, this is the first work on model-free GR for LRL in the feature space of generic deep RL agents. 
% does not fulfil both properties simultaneously.
% Instead, we investigate model-free generative replay as an alternative approach for such domains. It has two major components: i) A generative model that captures the distribution over the observations $p(o)$ when following previous policies. We impose no restrictions on the sampled observations, they can be related to arbitrary states. ii) A policy $\pi_s(o)$ that maps observations to a distribution over actions. The policy $\pi_s$ is what is evaluated in the evaluation blocks (EBs).
% The model-free view unifies the generative replay formulation for lifelong RL with lifelong supervised learning, potentially leading to agents that can tackle both kinds of learning problems.
% A small modification to the VAE is introduced: during sampling we generate an observation and perform an optional additional forward pass through the VAE (``Loop-VAE''), which has a sharpening effect on the generated observation.
%where maximizing the log-likelihood $\ln p(x|z)$ is equivalent to minimizing the mean squared error between the input $x$ and its reconstruction $\hat{x}$ output by the decoder, and $D_{KL}[q(z|x)||p(z)]$ is the KL-divergence between the distribution of the encoder and the prior on $z$.

==> SRI CoLLA 2022 L2M Paper Revised/technical.tex <==

\section{Hidden Replay for Lifelong RL}
\label{sec:model-free-generative-replay}
This section introduces our core contribution of wake-sleep training combined with model-free GR of latent representations. We also explore two other GR architectures along the way. 
 %One of the ways that lifelong RL differs from supervised continual learning is the lack of ground truth in any given task. In lifelong RL, the agent must improve its policy ``on-task'', and deal with two distinct sources of drift: change of task and change in policy within task. 
  %   \note{Suggestion: Denote in the pseudocode ``if using ER'', ``if using RaR'', and add the RaR to this pseudocode. RaR is generic to choice of M12/M15/M18 because the training is on observation-action pairs. Still unclear what the loss function is for these ER etc.}
% \note{ZACH TODO pseudocode to describe the flow in the architecture diagram}
    % \note{Suggestion: Add line numbers}
 %    \note{Maybe introduce a subroutine called ``GetSleepBatch'' and use it in sleep phase. In a separate pseudocode define ``GetSleepBatch'' in terms of ER, RaR and GR in there (in a way generic to M12/M15/M18).}
  % \note{Suggestion: Denote in the pseudocode ``if using ER'', ``if using RaR'', and add the RaR to this pseudocode. RaR is generic to choice of M12/M15/M18 because the training is on observation-action pairs. Still unclear what the loss function is for these ER etc.}
% \note{Suggestion: Add line numbers}
% \note{Maybe introduce a subroutine called ``GetSleepBatch'' and use it in sleep phase. In a separate pseudocode define ``GetSleepBatch'' in terms of ER, RaR and GR in there (in a way generic to M12/M15/M18).}
% \end{wrapfigure}
 % \begin{wrapfigure}{R}{0.5\textwidth}
%   \begin{minipage}{0.5\textwidth}
%     \begin{algorithm}[H]
%       \caption{Wake-Sleep Training in the Hidden Replay model \ref{}.}
%       \label{alg:hidden_replay}
%     \begin{algorithmic}[1]
%       \STATE {\bfseries Iterates:} Generator $g_s^t$, sleep policy $\pi_{s}^t$, wake policy $\pi_{w}^t$
%       % , Sleep frequency $K$, \# sleep iterations $N$
%       % \STATE Initialize $M$; set $B$ to empty; \# environment steps since last sleep $L=0$; current advice probability $\pi = 0$\\
%     	   \FOR{$t=1,2,\ldots$}
%     	   % \STATE Initialize task learner $T$
%     	   % \REPEAT
%     	   \FOR[Wake Phase]{$K$ times}
%     	       %\STATE{\# Take advice from sleep agent with probability $p_\text{advice}$}
%     	       % $ and from current wake agent with probability (1-$\pi$)}}
%     	       \STATE Let $a = \pi_s^t(o)$ w.p. $p_{\text{advice}}$, else $a = \pi_w^t(o)$
%     	       %\STATE{Execute $a_s$ w.p. $p_{\text{advice}}$ else execute $a_w$}
%     	       \STATE{Sample action from $a$}
%     	       \STATE{Add transition $(o, a)$ to wake buffer $b_w^t$}
%     	       \STATE{Update wake policy $\pi^t_w$.}
%     		   \STATE{Decay $p_\text{advice}$}
%     		   % \STATE{Store batch of observation-action pairs in buffer $B$}
%     		   %\STATE{$L = L + 1$}
%     		   %\STATE{$\pi = \max(\pi-D, \pi_{min})$}
%     	   % \ENDWHILE
%     	   \ENDFOR\\ %{$L==K$}\\
%     	   % \STATE{Create copy $g_s^t$}
%     	   \FOR[Sleep Phase]{$N$ iterations}
%     		   \STATE{Sample batch $B$ from $b_w^t$ (c.f.\! Line 6).} 
%     			 \STATE Sample batches $O_s^t \sim g_s^t$
%     			 \STATE Pseudo-label $A_s^t = \pi_s^t(O_s^t)$
%     			 \STATE Let $D = B \cup (O_s^t, A_s^t)$
%     			 \STATE Minimize $\mathcal{L}_{VAE}(g_s^{t+1}) + \alpha\mathcal{L}_{xent}(g_s^{t+1}, \pi_s^{t+1})$ on $D$
%     		\ENDFOR\\
    	 %     		 %\STATE{$t=t+1$}
%     	 \ENDFOR
%     \end{algorithmic}
%     \end{algorithm}
%     \end{minipage}
%     \note{Suggestion: Denote in the pseudocode ``if using ER'', ``if using RaR'', and add the RaR to this pseudocode. RaR is generic to choice of M12/M15/M18 because the training is on observation-action pairs. Still unclear what the loss function is for these ER etc.}
%     \note{Suggestion: Add line numbers}
%     \note{Maybe introduce a subroutine called ``GetSleepBatch'' and use it in sleep phase. In a separate pseudocode define ``GetSleepBatch'' in terms of ER, RaR and GR in there (in a way generic to M12/M15/M18).}
% \end{wrapfigure}
 The fundamental tradeoff in lifelong learning is between \emph{plasticity}, i.e.\!, learning the current task, and \emph{stability}, i.e.\!, remembering past tasks.
We address this tradeoff in lifelong RL by employing an approach that alternates between two distinct phases \citep{raghavan2020lifelong}.
%During the \emph{wake phase}, a plastic \emph{wake policy} $\pi_w$ is optimized on the current task by interaction with the environment and using any off-the-shelf RL method. During the \emph{sleep phase}, data from the wake phase is consolidated into a stable \emph{sleep model} consisting of a \emph{sleep policy} $\pi_s$ and \emph{generative memory} $g_s$. 
%Since our approach is based on memory consolidation, we handle this issue in two separate phases \citep{raghavan2020lifelong}. 
In the wake phase, a \emph{plastic} wake policy $\pi_w$ is optimized for the current task by interaction with the environment and using any off-the-shelf RL method.
Transition tuples are collected during training and stored in a buffer (see Alg. \ref{alg:wakesleep}); each tuple contains $(o, r, a)$, the observation $o$, reward for the previous action $r$, and the policy output $a$ (e.g., the policy logits or one-hot encoded action).
The sleep policy $\pi_s$ provides ``advice'' to explore the current task using the consolidated policy learned from all previous tasks.
Wake phase actions are selected according to a mixture of $\pi_w$ and $\pi_s$, the probability of choosing an action from $\pi_s$ decaying to 0 over time.
We use an off-policy RL algorithm such as VTrace \citep{espeholt2018impala} to accommodate this off-policy action selection in the optimization of $\pi_w$.

In the sleep phase, the \emph{stable} sleep policy $\pi_s$ is optimized with the objective of incorporating new knowledge (the action selection in the wake buffer) while retaining current knowledge. 
Similar to generative replay in supervised learning, augmented dataset(s) are created by combining wake transitions with tuples from the generative model $g_s$ and pseudo-labelled by the sleep policy. 
This form of replay is model-free because it does not learn the POMDP dynamics and reward and does not generate and replay temporal trajectories.  
%. Our method performs memory consolidation by 
% (Section~\ref{sec:model-free-generative-replay}).
%to generate simulated transition tuples from previous tasks to augment the real transitions in the wake buffer. 
% The sleep models $\pi_s$ and $g_s$ are then trained on the augmented data; the policy is trained via distillation \citep{rusu2015policy}. and generative memory $g_s$ are o
The sleep policy and the generative model are  jointly trained.
The sleep policy is trained to minimize $\mathcal{L}_{xent}$, a standard cross-entropy loss between the outputs (logits) of $\pi_s$, treating the replay augmented dataset as the ground truth. 
The generative model is trained using the combined dataset and the standard VAE loss (Eq. \ref{loss:vae}). 
 The description so far is easily applied to veridical replay, i.e.\!, when generative modelling and replay occurs in the original observation space of the MDP, but this is undesirable as discussed before. The design choice of whether the input or hidden space is replayed distinguishes the model implementations (Alg. \ref{alg:wakesleep} vs Alg. \ref{alg:hidden_replay}, and models in Fig. \ref{fig:all_replay_archs}) from each other. 

   \begin{minipage}{0.49\textwidth}
% \begin{wrapfigure}{R}{0.5\textwidth}
\begin{algorithm}[H]
   \caption{Wake-Sleep Training in the Sequential and Two-Headed models.} % \hyperlink{text:sequential}{Sequential} and \hyperlink{text:twoheaded}{Two-Headed} models.}
   \label{alg:wakesleep}
\begin{algorithmic}[1]
   \STATE {\bfseries Iterates:} Generator $g_s^t$, sleep policy $\pi_{s}^t$, wake policy $\pi_{w}^t$, wake buffer $b^t_w$
   % , Sleep frequency $K$, \# sleep iterations $N$
   % \STATE Initialize $M$; set $B$ to empty; \# environment steps since last sleep $L=0$; current advice probability $\pi = 0$\\
	   \FOR{$t=1,2,\ldots$}
	   % \STATE Initialize task learner $T$
	   % \REPEAT
	   \FOR[Wake Phase]{$K$ times}
	        \STATE{Sample observation $o$ and reward $r$ from current task}
	       %\STATE{\# Take advice from sleep agent with probability $p_\text{advice}$}
	       % $ and from current wake agent with probability (1-$\pi$)}}
	       \STATE Sample $a \sim \pi_s^t(o)$ w.p. $p_{\text{advice}}$, else $a \sim \pi_w^t(o)$
	       %\STATE{Execute $a_s$ w.p. $p_{\text{advice}}$ else execute $a_w$}
	       % \STATE{Sample action from $a$}
	       \STATE{Add transition $(o, r, a)$ to FIFO wake buffer $b_w^t$}
	       \STATE{Update wake policy $\pi^t_w$ on current task reward using $b^t_w$}
		   \STATE{Decay $p_\text{advice}$}
		   % \STATE{Store batch of observation-action pairs in buffer $B$}
		   %\STATE{$L = L + 1$}
		   %\STATE{$\pi = \max(\pi-D, \pi_{min})$}
	   % \ENDWHILE
	   \ENDFOR\\ %{$L==K$}\\
	   % \STATE{Create copy $g_s^t$}
	   \FOR[Sleep Phase]{$N$ iterations} 
		   \STATE{Sample batch $B$ from $b_w^t$ (c.f.\! Line 6).} 
			 \STATE Sample batches $O_s^t \sim g_s^t$
			 \STATE Pseudo-label $A_s^t = \pi_s^t(O_s^t)$
			 \STATE (GR Buffer) $D = B \cup (O_s^t, A_s^t)$
			 \STATE Minimize $\mathcal{L}_{VAE}(g_s^{t+1}) + \alpha\mathcal{L}_{xent}(g_s^{t+1}, \pi_s^{t+1})$ on $D$
		\ENDFOR\\
		 %\STATE{$t=t+1$}
	 \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
    \begin{algorithm}[H]
       \caption{Wake-Sleep Training in the  Hidden Replay model.} % \hyperlink{text:hidden}{Hidden Replay} model.}
       \label{alg:hidden_replay}
    \begin{algorithmic}[1]
       \STATE {\bfseries Iterates:} Generator $g_s^t$, sleep policy $\pi_{s}^t$, wake policy $\pi_{w}^t$, wake buffer $b^t_w$, random replay buffer $b^t_r$
       % , Sleep frequency $K$, \# sleep iterations $N$
       % \STATE Initialize $M$; set $B$ to empty; \# environment steps since last sleep $L=0$; current advice probability $\pi = 0$\\
    	   \FOR{$t=1,2,\ldots$}
    	   % \STATE Initialize task learner $T$
    	   % \REPEAT
    	   \FOR[Wake Phase]{$K$ times}
    	       %\STATE{\# Take advice from sleep agent with probability $p_\text{advice}$}
    	       % $ and from current wake agent with probability (1-$\pi$)}}
       	        \STATE{Sample observation $o$ and reward $r$ from current task}
    	       \STATE Sample $a \sim \pi_s^t(o)$ w.p. $p_{\text{advice}}$, else $a \sim \pi_w^t(o)$
    	       %\STATE{Execute $a_s$ w.p. $p_{\text{advice}}$ else execute $a_w$}
    	       % \STATE{Sample action from $a$}
    	       \STATE{Add transition $(o, r, a)$ to wake buffer $b^t_w$}
    	       \STATE{Update wake policy $\pi^t_w$ on current task reward using $b^t_w$}
    		   \STATE{Decay $p_\text{advice}$}
    		   % \STATE{Store batch of observation-action pairs in buffer $B$}
    		   %\STATE{$L = L + 1$}
    		   %\STATE{$\pi = \max(\pi-D, \pi_{min})$}
    	   % \ENDWHILE
    	   \ENDFOR\\ %{$L==K$}\\
    	   % \STATE{Create copy $g_s^t$}
    	   \FOR[Sleep Phase]{$N$ iterations}
    		   \STATE{If ER: Batch $B \sim b^t_w$ (c.f.\! Line 6).} 
    			 \STATE{If GR: Feature batches $H^t_s \sim g_s^t$}
    			 \STATE{If GR: Pseudo-label $A^t_s \sim \pi_s^t(H_s^t)$}
    			\STATE{If RaR: $b^t_r = b^t_r \bigcup b^t_w.sample(K)$}
    			\STATE{If RaR: $D_r \sim b^t_r$}
    			 \STATE Minimize $\mathcal{L}_{VAE}(g_s^{t+1}) + \alpha\mathcal{L}_{xent}(g_s^{t+1}, \pi_s^{t+1})$ on $(H^t_s, A^t_s)$ and end-to-end minimize (including feature extractor) the same loss on observation-action pairs in $B \bigcup D_r$
    		\ENDFOR\\
    		 %\STATE{$t=t+1$}
    	 \ENDFOR
    \end{algorithmic}
    \end{algorithm}
    \end{minipage}
    \hfill

%We show experimentally that sleep can occur on an arbitrary schedule (not necessarily at task changes) without degrading performance, and in Section \ref{sec:self-monitoring}, we investigate triggering sleep adaptively based on detecting feature drift. 

%In the basic version of wake-sleep, the wake model is not influenced by the sleep model, thus unable to leverage previously learned policies to an unseen but similar task (for jump start). We incorporate a form of ``advice'' within the wake phase, where $\pi_s$ influences the exploration of the current task during wake. We use off-policy RL for optimizing $\pi_w$. 
% A general wake-sleep cycle is shown in Algorithm \ref{alg:wakesleep}.

%The wake agent shares knowledge with the sleep agent by training the sleep agent to mimic the actions of the wake agent via a policy distillation loss. %In our StarCraft-2 experiments, this involves minimizing the cross-entropy between the logits of the wake agent and logits output by the sleep agent. In the Minigrid experiments, this involves minimizing the cross-entropy between the selected actions of the wake agent and actions selected by the sleep agent.
%The sleep agent is also capable of sharing information with the wake agent via ``advice'' by sampling the policy of the sleep agent instead of the wake agent's policy with some (generally linearly) decaying probability during wake. This decaying advice setting acts as an indirect way of forcing the wake agent to imitate the policy of the sleep agent until it learns to adapt to the current task.

% In our experiments, we sleep multiple times during the same task as well as at task changes. This results in an iterative policy distillation procedure where the sleep agent must not only deal with drifts in policy distribution caused by changes in task, but also distills knowledge of policies for the same task at different times, i.e., it begins by distilling sub-optimal policies of the task and as the wake agent improves, it distills increasingly better policies. %This demonstrates that our framework is capable of distilling off-policy knowledge in addition to off-task knowledge.

% \subsection{Model-Free Generative Replay}
% \label{sec:model-free-generative-replay}

% \note{introduce replay, generative replay, experience replay, its use in continual and lifelong learning, but not so much in RL}


\begin{figure}[t]
\centering
\includegraphics[width=0.92\textwidth]{graphics/updates_archs_2.png}
% \caption{We investigate three replay architectures for model-free generative replay. The red dashed arrows denotes sampling steps starting from the VAE to generate labelled actions. The black arrows denote the forward pass. \textbf{Top:} Sequential Replay Architecture; \textbf{Middle:} Two-Headed Replay Architecture; \textbf{Bottom:} Hidden Replay Architecture. \note{Show buffers esp. random replay}}
\caption{We investigate three replay architectures for model-free generative replay (sleep phase). The red dashed arrows denotes sampling steps starting from the VAE to generate labelled actions. The blue dashed arrows show how the various replay buffers are sampled and  fed into the sleep model during training. The black arrows denote the forward pass. \textbf{Top:} Sequential Replay Architecture; \textbf{Middle:} Two-Headed Replay Architecture; \textbf{Bottom:} Hidden Replay Architecture.}
% \note{$\checkmark$ Show buffers esp. random replay}}
% \note{Replace "Generative Replay" with "Generative Replay Buffer". Remove "Sample" except from VAE, no need sample for ERB and RaRB.}
% \note{Worth noting that all architectures optimize the same loss function specifically the linear combination of VAE losses and policy distillation loss.}
% \note{ERROR: Fig 1 bottom right box should not say ``Decoded Observations'', this should be ``Decoded Features''.}
\label{fig:all_replay_archs}
\end{figure}


%As mentioned, we retain current knowledge using model-free generative replay in conjunction with policy distillation. Experience replay (also known as rehearsal) is known to be an effective approach to lifelong and continual learning. 
%\note{this is the place to define loop vae if you need it}
%The actions are sampled on-policy and are typically made available via a replay buffer in RL implementations. 
%The policy network us  these actions come from , given observations $X$ (which might be sampled from real data or generated by the generative model), we use deep neural networks that are trained to imitate the policy (output actions $Y$) of other agents when presented with the same inputs via policy distillation \citep{rusu2015policy}. Policy distillation involves training the student policy network by minimizing the cross-entropy between either the logits or discrete actions of the student and teacher networks. 
%In the context of wake-sleep phases (Algorithm \ref{alg:wakesleep}), the wake phase provides a moving target for the current task via the updated policy $\pi_w^{t+1}$ and a replay buffer of $(o, a)$ tuples. % observed while training $\pi_w^{t+1}$. 
% Generative replay is used in the sleep phase to augment this data with tuples  $(O_s^t, A_s^t)$, where $O_s^t \sim g_s^t$ and $A_s^t = \pi_s^t(O_s^t)$. 
% These generated samples augment the samples from the wake phase available in the replay buffer $b_w^t$.
%Generated data sampled from the VAE is labeled by the sleep policy $\pi_s^{t}$.
% The total loss for sleep training is a weighted sum of the VAE loss and distillation loss and results in an updated sleep policy $\pi_s^{t+1}$ and generator $g_s$.

% \begin{align}
% \label{eq:complete_eqs}
% \pi_w^{t+1}, b_w^{t+1} &= \text{Wake}(\pi_w^t, \pi_s^t), \text{where $b$ is the replay buffer} \\ 
% \text{Sampling: } O_s^t &= g_s^t(Z), \text{where } Z \sim N(0, \mathbf{I})\\
% \text{Pseudo-label: } A_s^t, Y_s^t &= \pi_s^t(O_s^t)\\
% \pi_s^{t+1}, g_s^{t+1} &= \text{Sleep}(O_s^t \parallel A_s^t \parallel Y_s^t, b_w^{t+1}) \\
% \text{where sleep minimizes} & \min \mathcal{L}_\text{VAE} + \alpha\mathcal{L}_\text{distillation}
% \mathcal{L} = \mathcal{L}_{VAE} + \alpha\mathcal{L}_{distillation}
% \label{eq:gen_replay_loss}
% \end{align}
%Note that the pseudo-labels consist of the logits output by the policy applied to the generated observations.

%\note{needs to mention that pseudo label we take the full logits and not just the top 1}
% As mentioned previously, model-free generative replay treats each observation independent of the others; i.e., we do not need to distill entire trajectories and the data in a training batch can be off-policy and does not even need to belong to the same task.

%There are many possible neural architectures for sleep, differing on the combination of the VAE and policy. Algorithm \ref{alg:wakesleep} shows the pseudocode for model-free generative replay when the VAE samples raw observations. In the next section, we show that the VAE can operate on intermediate representations rather than raw observations.

%\begin{wrapfigure}{r}{0.40\textwidth}

% \subsection{Model-Free Generative Replay Architectures (Sleep Phase)}

We compare three replay architectures that we denote Sequential, Two-Headed, and Hidden Replay (shown in Fig. \ref{fig:all_replay_archs}). Each architecture is a specific arrangement of the following three components: a feature extractor, a VAE, and a policy network. The feature extractor maps raw image-like observations to feature vectors using a convolutional neural network (CNN) or a multi-layered perceptron. The policy network is dependent on the action space, e.g.,  in our experiments we utilize a convolutional architecture to output spatial actions.

In the \hypertarget{text:sequential}{\textbf{Sequential}} architecture (Fig.~\ref{fig:all_replay_archs}, Top), the VAE is upstream of the policy network, and the sleep policy $\pi_s$ operates on the VAE reconstruction rather than the true observation. This architecture is similar to the one proposed in \citet{atkinson2021pseudo}.
%Each observation is first passed through the encoder and decoder to obtain its reconstruction. %The reconstruction is then fed through the feature extractor, and the extracted features are then passed to the policy network. 
During sleep (following the red dashes in Fig.~\ref{fig:all_replay_archs}, Top), sampled latent vectors are decoded to observations that are then labelled by the policy. We hypothesize that the sequential architecture tends to map observations for which the policy chooses similar actions to generic reconstructions. We found that this method produces blurry reconstructions for image-like observations. % where loss of some important information can result in under-performing policies compared to single-task experts.
% by sampling from the decoder. 
%In our experiments, we employ a ``loop-vae'' style generation process where the generated samples make an additional pass through the encoder-decoder. We found this improves the quality of the reconstructions, which ultimately improves the lifelong learning metrics. Once a set of generated samples is obtained, action labels are assigned to these samples by passing them through the feature extractor-to-policy network portion of the architecture. The generated samples are mixed with observation-action pairs drawn from an experience replay buffer constructed from the previous wake cycle (consisting of data generally from only the current task), and this data is jointly passed through the entire model. The model is then trained on the loss discussed in the previous section.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.95\textwidth]{graphics/one_stream_model.png}
% \caption{Sequential architecture variant of model-free generative replay: The image gets passed through the generative model (VAE) and then the reconstruction is used as input to the policy network.}
% \label{fig:sequential_arch}
% \end{figure}
% The rationale behind the sequential architecture is by passing the real data and generated data through the encoder-decoder before passing it to the policy network, the data gets projected into a space better suited for the policy network; i.e., we hypothesize that it learns to map to generic observations that are more easily usable by the policy network. In practice, for image-like representations, we found that this method produces blurry reconstructions where some important information can lost before arriving at the policy network resulting in under-performing policies compared to single-task experts.

The \hypertarget{text:twoheaded}{\textbf{Two-Headed}} architecture (Fig.~\ref{fig:all_replay_archs}, Middle) decouples the decoder/generator from the policy network. Each observation (real or generated) is passed through the feature extractor. The features are then separately passed through the VAE and the policy network. Our experiments showed improved visual reconstructions (see Appendix \ref{sec:reconstructions_app}) due to separation of the influence of the policy on the VAE decoder. However, sampling in this architecture requires two forward passes as shown in the figure (once to decode an observation and once to label it). 

Alg. \ref{alg:wakesleep} shows the data flow that is common between these two architectures that perform veridical replay, i.e.\!, the VAE posterior is a density over raw and complex perceptual space. The training is wasteful because the wake policy $\pi_w$ has already learned an effective feature extractor, and latent-to-action partition that works well for the current task (solved in wake phase). The sleep phase in veridical replay does not utilize these learned features and tries to re-learn them, whereas deep RL (as in wake phase) is effective at learning representations to map raw percepts to actions.   

% Once again, generated observations are sampled from the decoded in a ``loop-VAE'' style and are mixed with the replay buffer from the wake data. This mixed data is then used for training the sleep model.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.95\textwidth]{graphics/two_stream_model.png}
% \caption{Two-headed architecture variant of model-free generative replay: The network still reconstructs observations, but the skill model is disconnected from the policy model.}
% \label{fig:two_headed_arch}
% \end{figure}

% \setlength\intextsep{0pt}
\setlength{\columnsep}{5pt}%
\begin{wrapfigure}{R}{0.35\textwidth}
\centering
\includegraphics[width=0.35\textwidth, keepaspectratio]{graphics/hidden_replay_partitioning.png}
\vspace{-0.75cm}
\caption{Hidden replay prevents drift in the features-to-action
mapping from the latent vector space of a deep RL agent (Minigrid tasks). Colors represent actions; $\times$s: drawn from the random replay buffer, $\bullet$: drawn from wake buffer; $\star$: sampled via generative replay.}
\vspace{-0.75cm}
\label{fig:hidden_replay_partitioning}
\end{wrapfigure}

The final architecture we consider is inspired by the success of \hypertarget{text:hidden}{\textbf{Hidden Replay}} in class incremental learning \citep{van2020brain} and its connection to biology. This architecture (Fig.~\ref{fig:all_replay_archs}, Bottom) generates feature vectors directly rather than observations. Sampling features instead of image-like observations benefits from dimensionality reduction. Reconstructing or generating complex image observations is hard and requires increasingly complex generative models \citep{van2017neural,van2016conditional,razavi2019generating}. In RL, especially when working with ``symbolic'' (semantic) (as opposed to ``perceptual'' (RGB)) observations, changing a small detail of the observation can change the optimal action drastically. Observations might be better separated in feature space, and thus, the sleep policy could be less sensitive to an imperfect decoder. In addition, in contrast to the two-headed architecture, the feature extractor does not need to be run when sampling. 
%sampling and labelling only use one pass effectively, because the feature extractor (usually a heavy CNN) does not need to be run on sampled features. 

For example, when faced with new tasks that require new actions to be taken, hidden replay can learn to add a new action partition to the feature space while rearranging the existing feature space in a manner that preserves partitioning needed to solve previous tasks. Empirically, we observe a clean partition of the feature space according to the optimal action. Even though samples and reconstructions are not perfect, they fall within the same action partition (Fig.~\ref{fig:hidden_replay_partitioning}) as the ground truth. These representations may allow for knowledge transfer between tasks because tasks requiring similar actions can potentially efficiently be mapped into the existing feature space, but validating this requires further studies. % or less interference when learning new tasks.

% When a new task appears that requires a new action partition, it should be able to %exploit the reserved space to more efficiently consolidate the latest wake policy with %the existing sleep policy.
% In this sense, hidden replay is similar to weight imprinting \citep{qi2018low}. 

% jh: Not sure this statement is empirically supported?
%Finally, by forcing the model to reconstruct features from previous tasks, the model is forced to reserve portions of the current feature space for specific tasks/actions. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.95\textwidth]{graphics/hidden_replay_model.png}
% \caption{Hidden replay architecture variant of model-free generative replay: The architecture is similar to the two-stream network, but the generator reconstructs the latent features from the feature extractor instead of the observations.}
% \label{fig:hidden_replay_arch}
% \end{figure}

%First, sometimes observations are reconstructed with missing important details. F the policy network might not be robust enough and could select a bad action. 

% \note{``These are accumulated over time by sampling from all replay
% buffers'' - means what? All replay buffers over lifetime, not over generative and wake buffers - right? As in, the random replay buffer is a union of random subsample of wake buffer? EDIT: Subsampling from generated data would be silly and already done by the generative replay (GR). Now this is abundantly clear from the updated Figure 1. Presumably RaR can be added in M12 and M15 also, but it is besides the point. I guess your comparison experiment between replay types used M18 in minigrid uniformly.}

Hidden replay is not without limitations because GR samples are in terms of features without the corresponding observations. This V-shape in the training graph (blue lines in Fig. \ref{fig:all_replay_archs}, Bottom) can cause the feature extractor to drift over time or collapse to a mode (e.g., map all observations to the same feature vector). 
As new tasks are encountered, this would cause sampled features %from previous tasks 
to not align with the features mapped by the policy and VAE components. 
% of this model, which receive additional supervision from generative memory. 

To limit feature drift, we store a small (typically $K < 1\%$ of the experience replay buffer) set of raw observations paired with actions in a separate buffer. We denote this RaR (for  ``random replay'' buffer). These are accumulated over the lifetime of the agent from all wake replay buffers $b^t_w$ (although a more sophisticated exemplar selection \citep{rebuffi2017icarl,mi2020ader} is also possible). We observed that replaying a few random examples results in less feature drift between task changes (See Appendix ~\ref{sec:justification_of_exemplars} for an ablation). In our experiments, we found that saving 96 random samples per sleep was sufficient to alleviate feature drift in the \SC{} domain and saving 256 random samples per sleep was sufficient for the Minigrid domain. The complete data flow for hidden replay for LRL is shown in Alg. \ref{alg:hidden_replay}, where the design choice of combinations of ER, GR, and RaR buffers are ablated in our experimental ablations. 

% \note{Moved justification of exemplars to appendix with reference here (when we introduce the idea of combining gen replay + exemplars) as this is an important finding, but not a core theoretical contribution of the paper. Can add back to main results if need be.}
% \note{I think some of these need to be brought back to the experiemtns}

% It should also be noted that we do not employ a ``loop-VAE'' style generation process for hidden replay. Instead, we sample from the decoder and do not re-pass generated observations through the encoder-decoder.
% \note{check for consistency of SC2 vs SC-2 vs SC-II}

% \section{\sout{Creating Starcraft Agents using Lifelong Learning Components}}
% \label{sec:integration}
% % Extending the System with Other Lifelong Learning Components}

% %\note{Move to Sec 5.2 and break out}

% \sout{In this section, we focus on improving the lifelong RL metrics for SC-2. 
% While the wake-sleep mechanism and model-free generative replay show promising results, we continue to see evidence of catastrophic forgetting via low PM (Section \ref{sec:architecture_comparison_experiments}). 
% We explore the integration of lifelong learning components within the context of  wake-sleep, and show the framework to be sufficiently expressive. Each such component is motivated by recent work in continual learning. 
% These extensions include automatically triggering sleep via recent work in changepoint detection \citep{faber2021watch}, compression of experiences in the replay buffer \citep{hayes2019remind}, an SC-2-specific prioritized replay mechanism, and representation learning from RGB-observations via unsupervised and self-supervised learning. In each case, the lifelong learning metrics are either improved or unaffected by the addition of each component.
% Since deep learning in SC-2 is computationally demanding, we released a dataset  generated by single task expert policies in order to enable our multi-institution  collaborative effort, and we make it publicly available for future research.}

% \subsection{\sout{Handling Task Interference via Eigentasks}}

% %\note{check that authorship is not given away by saying eigentask is our prior work} 
% \sout{The success of our approach depends on the capacity of the VAE and policy networks to generate samples from a wide range of tasks. Generative replay can have difficulties with highly interfering tasks where similar observations require different actions. Prior work overcomes this issue by learning a mixture of VAE-policy pairs, known as \emph{Eigentasks} \citep{raghavan2020lifelong}. The mixture can capture mixture distributions in both the observation space and the policy space (i.e., concept drift). Eigentasks are designed to partition the joint observation-action space in such a way that observations that rely on similar actions are assigned to the same eigentask. To learn to partition the data, the eigentask framework combines the mixture-of-experts \citep{tsuda_modeling_2020} concept with generative replay. The objective for eigentask learning is our basic loss function (in Alg.~\ref{alg:wakesleep}) averaged over the mixture probabilities, %The objective for eigentask learning is our basic loss function (Eq.~\ref{eq:complete_eqs}) averaged over the mixture probabilities,
% \begin{equation}
% \small
% \min E_\tau(X) [\mathcal{L}_{\text{VAE}} + \alpha\mathcal{L}_{\text{dist}}], \text{where } \tau_i(x) = \sigma\Big(\frac{\Phi(z_i)}{\max_j \Phi_j(z_j)}\Big),
% \label{eq:eigtask_loss}
% \end{equation}
% where $\alpha$ is a trade-off parameter, $z$ is the latent vector of the VAE, $\Phi$ is the density of standard gaussian, $\sigma$ denotes softmax, and $\tau$ captures the likelihood ratio between VAEs.}
% % An Eigentask is a tuple $E = (g, f)$ consisting of a generator $g(\epsilon)$
% % that defines a distribution over inputs $\mathcal{X}$ as a
% %function of random noise $\epsilon$,
% %and a skill $f : \mathcal{X} \mapsto Prob(\mathcal{Y})$ that maps inputs to outputs.
% %An Eigentask model consists of a set of Eigentasks $\mathcal{E}$ and a similarity function %$\tau: \mathcal{X} \mapsto\ Prob(\mathcal{E})$ whose
% %output is a probability vector over the $n$ eigentasks. In this work, $g$, $f$ and $\tau$
% %are parameterized by deep neural network models.

% %Given a dataset $\{X, Y\}$, 

% % \begin{equation}
% %     \tau_i(x) = \sigma\Big(\frac{\Phi(z_i)}{\max_j \Phi_j(z_j)}\Big) \label{eq:tau_latent}
% % \end{equation}
% % where subscript $i$ denotes eigentask $i$, $z$ is the latent vector of the VAE, $\Phi$ is the density of standard gaussian, $\sigma$ denotes softmax. 

% \subsection{\sout{Self-Monitoring for Sleep via WATCH}}
% \label{sec:self-monitoring}

% % NOTE: The LIFEWATCH paper is currently under review at IJCNN 2022. For now we can keep the reference to WATCH and add LIFEWATCH in the camera ready version if the paper is accepted in the meanwhile.

% %\note{it is not discovering just task change it is also discovering learning changes}
% %\note{Can't find any reference in the literature to a LIFEWATCH technique?}
% \sout{Up until now, sleep was triggered after a fixed number of interactions with the environment. This can be inefficient due to the overhead of sleep, and lead to reduced performance due to over emphasizing memory consolidation versus learning. We hypothesize that triggering sleep adaptively at opportune times will lead to better performance with less overhead. We apply an unsupervised change-point detection method \citep{faber2021watch} to the features extracted from SC-2 observations using a pre-trained VGG-16 model \citep{simonyan2014very}
% because (a) our setting does not assume knowledge of task changepoints, and (b) sleep can be beneficial even when the task has not changed, i.e. a significant change in the policy can cause it to visit novel states and observations. In principle, changepoint detection can be applied to episodic reward as well.  
% %can be used to automatically discovers transitions between tasks, which may trigger an \textit{adaptive sleep} before the scheduled sleep phase, allowing the system to consolidate knowledge without having to wait for a predefined number of steps. 
% %The proposed change point detection component analyzes features 
% Preliminary experiments showed that standard methods for change point detection like CUMSUM appear unreliable in the presence of  the high-dimensional features, whereas the recently proposed WATCH method \citep{faber2021watch} performs better.} 
% %that models an initial distribution over the data and monitors the distribution's behavior as new data points arrive. The Wasserstein distance $W_P$ is adopted to provide accurate and robust detection of change points in dynamic high-dimensional data. We calculate $W_P$ using the SAG approximated computational method as explained in \citet{hallin2021multivariate}. A significant advantage of our approach is that it compares two sets of points instead of working on the parameters of specific distributions. This mechanism allows to compare distributions of unknown types. 
% % PM and FTR while achieving similar BTR and RP.

% % The original formulation of the Wasserstein distance is intractable in nature. In our work, the Wasserstein distance $W_P$ is calculated using the SAG approximated computational method as explained in \citet{hallin2021multivariate}.

% % The input of the algorithm is a time series of data samples $\mathbf{I} = (I_1, I_2, \ldots, I_T)$, where each data sample is a $d$-dimensional vector: $I_t\in \mathbb{R}^d$. 
% % Our method learns a new representation of a distribution $D$ in an unsupervised manner using an initial set of data points. The method incrementally stores newly available samples in a buffer. Once the capacity of the buffer (controlled by a $\kappa$ parameter) is reached, the change detection procedure is activated. In this process, we collect newly arriving points in mini-batches  of length $\omega$ (sliding non-overlapping windows), and calculate the Wasserstein distance of every mini-batch $B$ with respect to $D$.
% % If the distance is lower than the desired threshold $\gamma$ (controlled by the $\epsilon$ parameter), we qualify $B$ as belonging to $D$. The threshold is determined as:
% % \begin{equation}
% %     \eta(D, \ \epsilon) = \ \epsilon \ \max_{B \in D}  \ W_A(B, D) .
% % \label{eq:threshold}
% % \end{equation}
% % Consequently, $D$ is updated to reflect the new data points. On the contrary, if the distance is higher than $\gamma$, we assume that the current mini-batch $B$ being analyzed belongs to a different distribution. Therefore, we annotate this point in time as a change point and start creating a new distribution to replace $D$.  Once $D$ reaches its storage capacity controlled by $\mu$, the oldest samples are removed to accommodate new ones, in order to keep an up-to-date representation of the distribution $D$.
% % A significant advantage of our approach is that it compares two sets of points instead of working on the parameters of specific distributions. This mechanism allows to compare distributions of unknown types, without limiting the scope to only the most popular ones, such as Normal distributions.

% % We compared the system with and without self-triggering sleep on two lifelong RL scenarios in the SC2 domain. Experimental results (Tables~\ref{tab:algo-M121518} and \ref{tab:self_triggering_sleep_comparison}), suggest that self-triggering sleep results in improved PM and FTR while achieving similar BTR and RP.

% \subsection{\sout{Improvements on Experience Replay}}

% \sout{Clever strategies for efficient management of replay buffers have been shown to improve supervised continual learning \citep{riemer2019scalable, wang2021acae} and lifelong RL \citep{caccia2020online,zhang2017deeper,schaul2015prioritized}.
% In contrast to prior work that rejects most transitions from being stored in the buffer, we explore two ideas that store all the transitions but in a highly compressed form, and prioritize the replay of certain transitions.}

% \textbf{\sout{Experience Compression via REMIND}}: 
% \sout{Compression allows a buffer of a given size to contain a larger number of transitions, increasing the chance of retaining diverse examples from different tasks. We use the REMIND \citep{hayes2019remind} method, based on Product Quantization (PQ) \citep{jegou2010product}, to compress the agent's observations before storing them in the replay buffer, allowing the system to store more samples. The agent observations are image-like \texttt{float32} tensors with $3$ channels, and thus each pixel occupies $96$ bits. In the compressed observation, each pixel is quantized to an 8-bit integer, a 24x reduction in size. The PQ model is pre-trained on observations collected while following a random policy on a subset of tasks that is disjoint from the set of evaluation tasks.}

% Iterative policy distillation requires storing a buffer of experiences from the wake phase to replay during sleep. This buffer must be large enough to contain a representative sample of all tasks encountered during the wake phase, but in real-world applications, the amount of memory available for the buffer may be limited. This motivated us to explore a mechanism for compressing the wake experience buffer to reduce its memory footprint.

% The experience compression subsystem uses elements from REMIND \citep{hayes2019remind}. REMIND uses Product Quantization (PQ) \citep{jegou2010product} on the feature representation computed by the first few layers of a neural network to efficiently encode input-output pairs. This compact encoding enables storing and replaying large memories of previous training instances, which has been shown to greatly reduce forgetting in supervised lifelong learning settings \citep{hayes2019remind}. In the current system, 

% Our implementation uses the \texttt{ProductQuantizer} class from the FAISS library \citep{johnson2019billion}. 

% \begin{table}[htp]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%         \hline
%          Scenario & Agent & PM & FT & BT & RP & SE \\
%          \hline
%           Pairwise & Eigentask Model & $-3.35$ ($ \pm 4.3$) & $1.45$ ($ \pm 0.4$) & $0.92$ ($ \pm 0.15$) & $1.12$ ($ \pm 0.21$) & $33.02$ ($ \pm 26.77$) \\
%          & Eigentask Model + REMIND & $-2.23$ ($ \pm 2.33$) & $1.58$ ($ \pm 0.22$) & $0.93$ ($ \pm 0.22$) & $0.97$ ($ \pm 0.13$) & $20.0$ ($ \pm 10.72$) \\
%          \hline
%           Alternating & Eigentask Model & $-8.44$ ($ \pm 5.35$) & $1.04$ ($ \pm 0.31$) & $0.81$ ($ \pm 0.13$) & $0.89$ ($ \pm 0.07$) & $6.08$ ($ \pm 1.74$) \\
%          & Eigentask Model + REMIND & $-6.51$ ($ \pm 4.58$) & $1.29$ ($ \pm 0.35$) & $0.78$ ($ \pm 0.2$) & $0.92$ ($ \pm 0.04$) & $5.71$ ($ \pm 1.67$) \\
%          \hline
%         Condensed & Eigentask Model & $-4.08$ ($ \pm 4.17$) & $1.52$ ($ \pm 0.25$) & $1.2$ ($ \pm 0.47$) & $1.1$ ($ \pm 0.2$) & $37.45$ ($ \pm 30.44$) \\
%          & Eigentask Model + REMIND & $-3.67$ ($ \pm 3.92$) & $1.5$ ($ \pm 0.18$) & $1.13$ ($ \pm 0.42$) & $1.11$ ($ \pm 0.18$) & $21.73$ ($ \pm 13.54$) \\
%          \hline
%     \end{tabular}
%     }
%     \caption{Comparison of the Eigentask model with and without a compressed wake buffer (REMIND). Results are averaged over 12 lifetimes and we also record the 95\% confidence interval according to the t-distribution.}
%     \label{tab:remind}
% \end{table}

% \textbf{\sout{Danger Detection for Prioritized Replay}}: 
% \sout{In addition to compression of experiences, we examine a novel form of prioritized experience replay \citep{schaul2015prioritized} based on detecting dead-end states. We hypothesize that increasing the lifetime of an agent by avoiding dead end states is a useful bias. 
% %Consider an SC-2 game involving force-on-force battles. States where units are in combat have a much greater impact on agent performance than states with no combat.
% %A significant portion of each trajectory provides little information for training because the units are not in combat. On the other hand, uniformly sampling experiences from such a biased buffer can cause overfitting and increase the time for learning. 
% The Danger Detector outputs a ``danger score'' of how likely the agent is to lose the battle from a given state. This score is used as a replay priority.
% The policy's actions in the battle change over time, making the danger detection task a continual learning problem. 
% We used Deep Streaming Linear Discriminant Analysis (DeepSLDA) \citep{hayes2019lifelong} for our danger detector.  
% % We continually train the danger detector in parallel with the RL policy. 
% At the end of each episode, we obtain ground truth of the result of the battle and continually update the danger detector. 
% %The observations and labels are fed to the danger detector in an online streaming learning fashion. 
% Deep SLDA works on top of a fixed feature extractor; we pre-trained a feature extractor based on the FullyConv architecture of \citep{vinyals2017starcraft} using data generated from STEs.}

% Rather buffer as the wake data experience buffer. Specifically, in the combat-related tasks of the SC2 domain, the agent frequently encounters dangerous states, which can lead to death and thus, under-exploration. We hypothesize that increasing the lifetime of an agent by avoiding dead end states is a useful bias for lifelong learning. Avoiding dead end states allows the agent to collect more data from learning experiences, increasing the length of episodes in combat tasks, and potentially improving the overall performance. To test this hypothesis, we created a Danger Detector subsystem which assigns a \textit{danger score} to current states. Dead end states prediction, or danger detection, can be seen as predicting the outcome of an ongoing battle. The goal is to predict if the agent units will eventually lose the current battle, giving the agent the opportunity to disengage from the fight and regroup, increasing its lifetime.

%The strategy of the reinforcent learner to address a battle changes in time, making the danger detection task a continual learning problem. 
%The strategy used by the policy to address a battle changes over time, making the danger detection task a binary classification continual learning problem. The score output by the danger detector is interpreted as the priority.  
% We used Deep SLDA~\citep{hayes2019lifelong} for our danger detector subsystem. Deep SLDA stores a set of running mean vectors for each class and a shared covariance matrix, and it classifies a new input by assigning it the label of the closest Gaussian in feature space. Deep SLDA works on top of a fixed feature extractor that it is pre-trained using a small set of data. For the SC2 case, we pre-trained the feature extractor (based on the FullyConv architecture of \citet{vinyals2017starcraft}) using data generated from expert agents. We continually train the danger detector in parallel with the RL policy. At the end of each episode, we obtain ground truth of the result of the battle. The frame data and labels are fed to the danger detector in an online streaming learning fashion following Deep SLDA.
% \note{expand SLDA first time}
% gather all of the episode's frames, and using a \textit{battle detector} pre-processing block, split these frames into battles with their corresponding label (lost or won battle). The frame data and labels are fed to the danger detector in an online streaming learning fashion following Deep SLDA. The danger detector learns to yield a score between 0 (won battle) and 1 (lost battle) for each frame. During inference, this score is used as an indicator of danger.
 
%This is done by a \textit{battle detector} pre-processing block which finds battle resets in each episode when there is a sudden increment of units between frames. 

% \subsection{\sout{Representation Learning for Generalization}}

% \sout{In earlier experiments, we assumed that the observations are hand-crafted representations provided by the PySC2 simulator. In practice, agents must learn a  representation from RGB percepts as tasks change over time. In this section, we consider unsupervised and self-supervised continual representation learning. }

% \sout{\textbf{Self-Taught Associative Memory} (STAM) \citep{smith2019unsupervised} was originally designed for the Unsupervised Progressive Learning \citep{smith2019unsupervised2} problem: an online representation learning problem in which the learner observes a non-stationary and unlabeled data stream. STAM learns patch-based features through online clustering of a stream of RGB image input (Section \ref{sec:stam_app}). The number of clusters increases over time, driven by a novelty detection mechanism that identifies when a new observation is significantly different from all current centroids. Additionally, STAM maintains a limited-memory collection of short-term centroids (can be forgotten) and long-term centroids (that are difficult to forget). Observations are represented via an embedding using a voting-based scheme over these centroids.}

%Applying STAM to the SC2 domain involves six steps: i) pre-processing of observations, which separates objects from background in the RGB observations, ii) patch-based feature extraction, iii) clustering of patches into centroids, iv) detection of novel inputs in a streaming setting to identify new centroids, v) learning using dual-memory organization which manages centroids stored in short- and long-term memory, vi) embedding observations via a vote-based method on the centroids.

%\note{Not sure if this is okay for describing the STAM algorithm? Might need feedback from whoever worked on STAM}

%\note{expand STAM for first time}

%includes a brain-inspired dual-memory hierarchy (short-term versus long-term) that enables the conservation of previously learned features (to avoid catastrophic forgetting) that have been seen multiple times at the data stream, while forgetting outliers. 

% For SC2, STAM operates over an image input in the form of a raw RGB frame from the simulation as opposed to the screen feature maps typically used for reinforcement learning. This presents a much more difficult, but also realistic challenge for both STAM and ultimately the reinforcement learning agent as well. A detailed explanation of how STAM is applied to SC2 can be found in Section \ref{sec:stam_app}, and a detailed description of the original STAM model can be found in \citet{smith2019unsupervised}.

% \sout{\textbf{Self-Supervised Representation Learning} (SSRL): 
% Motivated by recent work that representation learned using self-supervision auxiliary losses can boost lifelong learning performance~\citep{gallardo2021self}. The intuition is that features learned from an auxiliary losses generalize more than   features learned from task-specific losses, and therefore may be less vulnerable to forgetting. The representation is generated from RGB input from two SC-2 tasks, processed by a ResNet18~\citep{he2016deep}, then refined using Barlow Twins~\citep{zbontar2021barlow} self-supervised learning. We chose this approach by validating on object detection performance using Average Precision 50(AP50) as a metric within the SC-2 framework, finding that 1) the ImageNet1k pre-training was beneficial and 2) Barlow Twins outperformed other SSL methods such as MoCo-V2~\citep{chen2020improved} and SimCLR~\citep{chen2020simple}. Further details of this experiment appear in Section \ref{sec:barlow_app}.}

% We explore representations learned using self-supervision with a sub-system we refer to as \textit{Self-Supervised Representation Learning} (SSRL). The motivation for this sub-system comes from prior works, which have shown that self-supervision from auxiliary losses can boost lifelong learning performance~\citep{gallardo2021self}. The intuition is that features learned from an auxiliary loss are more generalized compared to features learned from prior task losses, and therefore may be less vulnerable to forgetting.

% We explore this idea by expanding the screen features used by the baseline SC2 system with features learned from self-supervised learning (SSL). The features are generated from a ResNet18~\citep{he2016deep} model pretrained on ImageNet-1k~\citep{deng2009imagenet}, then refined using Barlow Twins~\citep{zbontar2021barlow} SSL on RGB observations from two tasks. 

% Table~\ref{tab:ssrl_od} shows the evaluation of the SSL trained backbones used in the Object Detection pipeline. To ensure that other components of the pipeline(RPN, ROI pooling) do not mask the contribution of the backbone, we ran the experiments on three pipelines (C4, FPN and DC5) offered by Detectron2\citep{wu2019detectron2}.
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline Backbone/Pipeline & C4 & FPN & DC5 \\
%     \hline
%          Barlow Twins & 12.943 & 42.641 & 6.083 \\
%          MoCo & 6.083 & 43.110 & 6.675 \\
%          Barlow Twins, initialized with ImageNet & 9.382 & 44.325 & 7.841 \\
%          MoCo , initialized with ImageNet & 9.693 & 42.802 & 6.395 \\MoCo , initialized with ImageNet & 9.693 & 42.802 & 6.395 \\ 
%          ImageNet & 14.903 & 42.107 & 6.885 \\
%   \hline
%     \end{tabular}
%     \caption{Evaluation of SSL trained backbones using Object Detection as downstream task}
%     \label{tab:ssrl_od}
% \end{table}

% In this way, hidden replay is similar to weight imprinting \citep{qi2018low}. 

\textbf{Remark}: When applied to single task RL, our wake-sleep cycle resembles policy iteration interleaved with policy distillation steps, where each iteration $t$ produces an improved $\pi_w^t$ (nudge towards STE) that is then distilled into $\pi_s^t$. Wake experiences are gathered from the most recent sleep policy (``advice''), including from multiple sub-optimal policies similar in spirit to dataset aggregation in DAGGER \citep{ross2011reduction}. Similar to DAGGER, the consolidated policy is executed to sample next trajectories. Our supplementary experiments (Appendices \ref{sec:wake_additional_results} and \ref{sec:ste_additional_results})  show stable convergence of the wake-sleep cycle to optimal policies in single task training (convergence to STE). 
